Quantile-based fuzzy C-means clustering of multivariate time series: Robust techniques

Three robust methods for clustering multivariate time series from the point of view of generating processes are proposed. The procedures are robust versions of a fuzzy C-means model based on: (i) estimates of the quantile cross-spectral density and (ii) the classical principal component analysis. Robustness to the presence of outliers is achieved by using the so-called metric, noise and trimmed approaches. The metric approach incorporates in the objective function a distance measure aimed at neutralizing the effect of the outliers, the noise approach builds an artificial cluster expected to contain the outlying series and the trimmed approach eliminates the most atypical series in the dataset. All the proposed techniques inherit the nice properties of the quantile cross-spectral density, as being able to uncover general types of dependence. Results from a broad simulation study including multivariate linear, nonlinear and GARCH processes indicate that the algorithms are substantially effective in coping with the presence of outlying series (i.e., series exhibiting a dependence structure different from that of the majority), clearly poutperforming alternative procedures. The usefulness of the suggested methods is highlighted by means of two specific applications regarding financial and environmental series.

==> mybibfile.bbl.tex <==


%A


@article{abraham1989outlier,
	title={Outlier detection and time series modeling},
	author={Abraham, Bovas and Chuang, Alice},
	journal={Technometrics},
	volume={31},
	number={2},
	pages={241--248},
	year={1989},
	publisher={Taylor \& Francis}
}


@article{aghabozorgi2015time,
	title={Time-series clustering--a decade review},
	author={Aghabozorgi, Saeed and Shirkhorshidi, Ali Seyed and Wah, Teh Ying},
	journal={Information Systems},
	volume={53},
	pages={16--38},
	year={2015},
	publisher={Elsevier}
}


@inproceedings{agyemang2004lsc,
	title={Lsc-mine: Algorithm for mining local outliers},
	author={Agyemang, Malik and Ezeife, Christie I},
	booktitle={Proceedings of the 15th Information Resource Management Association (IRMA) International Conference, New Orleans},
	volume={1},
	pages={5--8},
	year={2004},
	organization={Citeseer}
}

@article{alonso2019clustering,
	title={Clustering time series by linear dependency},
	author={Alonso, Andr{\'e}s M and Pe{\~n}a, Daniel},
	journal={Statistics and Computing},
	volume={29},
	number={4},
	pages={655--676},
	year={2019},
	publisher={Springer}
}

@article{andersson2008does,
	title={Why does the correlation between stock and bond returns vary over time?},
	author={Andersson, Magnus and Krylova, Elizaveta and V{\"a}h{\"a}maa, Sami},
	journal={Applied Financial Economics},
	volume={18},
	number={2},
	pages={139--151},
	year={2008},
	publisher={Taylor \& Francis}
}


@article{arabie1981overlapping,
	title={Overlapping clustering: A new method for product positioning},
	author={Arabie, Phipps and Carroll, J Douglas and DeSarbo, Wayne and Wind, Jerry},
	journal={Journal of Marketing Research},
	volume={18},
	number={3},
	pages={310--317},
	year={1981},
	publisher={SAGE Publications Sage CA: Los Angeles, CA}
}



@inproceedings{awwad2008nonlinear,
	title={Nonlinear autoregressive moving average (NARMA-L2) controller for advanced ac motor control},
	author={Awwad, A and Abu-Rub, H and Toliyat, HA},
	booktitle={2008 34th Annual Conference of IEEE Industrial Electronics},
	pages={1287--1292},
	year={2008},
	organization={IEEE}
}

%B





@inproceedings{banerjee2010ecg,
	title={ECG feature extraction and classification of anteroseptal myocardial infarction and normal subjects using discrete wavelet transform},
	author={Banerjee, Swati and Mitra, Madhuchhanda},
	booktitle={2010 International Conference on Systems in Medicine and Biology},
	pages={55--60},
	year={2010},
	organization={IEEE}
}


@article{banerjee2013application,
	title={Application of cross wavelet transform for ECG pattern analysis and classification},
	author={Banerjee, Swati and Mitra, Madhuchhanda},
	journal={IEEE transactions on instrumentation and measurement},
	volume={63},
	number={2},
	pages={326--333},
	year={2013},
	publisher={IEEE}
}


@article{baragona2007outliers,
	title={Outliers detection in multivariate time series by independent component analysis},
	author={Baragona, Roberto and Battaglia, Francesco},
	journal={Neural computation},
	volume={19},
	number={7},
	pages={1962--1984},
	year={2007},
	publisher={MIT Press}
}


@article{bastos2014clustering,
	title={Clustering financial time series with variance ratio statistics},
	author={Bastos, Jo{\~a}o A and Caiado, Jorge},
	journal={Quantitative Finance},
	volume={14},
	number={12},
	pages={2121--2133},
	year={2014},
	publisher={Taylor \& Francis}
}

@article{basu2007automatic,
	title={Automatic outlier detection for time series: an application to sensor data},
	author={Basu, Sabyasachi and Meckesheimer, Martin},
	journal={Knowledge and Information Systems},
	volume={11},
	number={2},
	pages={137--154},
	year={2007},
	publisher={Springer}
}


@article{bauwens2006multivariate,
	title={Multivariate GARCH models: a survey},
	author={Bauwens, Luc and Laurent, S{\'e}bastien and Rombouts, Jeroen VK},
	journal={Journal of applied econometrics},
	volume={21},
	number={1},
	pages={79--109},
	year={2006},
	publisher={Wiley Online Library}
}


@article{battaglia2005outlier,
	title={Outlier detection and estimation in nonlinear time series},
	author={Battaglia, Francesco and Orfei, Lia},
	journal={Journal of Time Series Analysis},
	volume={26},
	number={1},
	pages={107--121},
	year={2005},
	publisher={Wiley Online Library}
}


@article{beggel2019time,
	title={Time series anomaly detection based on shapelet learning},
	author={Beggel, Laura and Kausler, Bernhard X and Schiegg, Martin and Pfeiffer, Michael and Bischl, Bernd},
	journal={Computational Statistics},
	volume={34},
	number={3},
	pages={945--976},
	year={2019},
	publisher={Springer}
}


@incollection{ben2003detecting,
	title={Detecting stable clusters using principal component analysis},
	author={Ben-Hur, Asa and Guyon, Isabelle},
	booktitle={Functional genomics},
	pages={159--182},
	year={2003},
	publisher={Springer}
}


@article{benkabou2018unsupervised,
	title={Unsupervised outlier detection for time series by entropy and dynamic time warping},
	author={Benkabou, Seif-Eddine and Benabdeslem, Khalid and Canitia, Bruno},
	journal={Knowledge and Information Systems},
	volume={54},
	number={2},
	pages={463--486},
	year={2018},
	publisher={Springer}
}


@article{bernardi2017multiple,
	title={Multiple risk measures for multivariate dynamic heavy--tailed models},
	author={Bernardi, Mauro and Maruotti, Antonello and Petrella, Lea},
	journal={Journal of Empirical Finance},
	volume={43},
	pages={1--32},
	year={2017},
	publisher={Elsevier}
}


@article{bensaid1996validity,
	title={Validity-guided (re) clustering with applications to image segmentation},
	author={Bensaid, Amine M and Hall, Lawrence O and Bezdek, James C and Clarke, Laurence P and Silbiger, Martin L and Arrington, John A and Murtagh, Reed F},
	journal={IEEE Transactions on fuzzy systems},
	volume={4},
	number={2},
	pages={112--123},
	year={1996},
	publisher={IEEE}
}
@article{bensaid1996validity,
	title={Validity-guided (re) clustering with applications to image segmentation},
	author={Bensaid, Amine M and Hall, Lawrence O and Bezdek, James C and Clarke, Laurence P and Silbiger, Martin L and Arrington, John A and Murtagh, Reed F},
	journal={IEEE Transactions on fuzzy systems},
	volume={4},
	number={2},
	pages={112--123},
	year={1996},
	publisher={IEEE}
}


@book{bezdek2013pattern,
	title={Pattern recognition with fuzzy objective function algorithms},
	author={Bezdek, James C},
	year={2013},
	publisher={Springer Science \& Business Media}
}

@article{blazquez2020review,
	title={A review on outlier/anomaly detection in time series data},
	author={Bl{\'a}zquez-Garc{\'\i}a, Ane and Conde, Angel and Mori, Usue and Lozano, Jose A},
	journal={arXiv preprint arXiv:2002.04236},
	year={2020}
}


@article{bollerslev1986generalized,
	title={Generalized autoregressive conditional heteroskedasticity},
	author={Bollerslev, Tim},
	journal={Journal of econometrics},
	volume={31},
	number={3},
	pages={307--327},
	year={1986},
	publisher={Elsevier}
}


@book{box2015time,
	title={Time series analysis: forecasting and control},
	author={Box, George EP and Jenkins, Gwilym M and Reinsel, Gregory C and Ljung, Greta M},
	year={2015},
	publisher={John Wiley \& Sons}
}



@inproceedings{boynton2013application,
	title={Application of nonlinear autoregressive moving average exogenous input models to geospace: advances in understanding and space weather forecasts},
	author={Boynton, RJ and Balikhin, MA and Billings, SA and Amariutei, OA},
	booktitle={Annales Geophysicae},
	volume={31},
	number={9},
	pages={1579--1589},
	year={2013},
	organization={Copernicus GmbH}
}

 
 @incollection{bradley2003financial,
 	title={Financial risk and heavy tails},
 	author={Bradley, Brendan O and Taqqu, Murad S},
 	booktitle={Handbook of heavy tailed distributions in finance},
 	pages={35--103},
 	year={2003},
 	publisher={Elsevier}
 }


@article{brigham1967fast,
	title={The fast Fourier transform},
	author={Brigham, E Oran and Morrow, RE},
	journal={IEEE spectrum},
	volume={4},
	number={12},
	pages={63--70},
	year={1967},
	publisher={IEEE}
}

%C


@article{cai2003simple,
	title={A simple diagnostic method of outlier detection for stationary Gaussian time series},
	author={Cai, Yuzhi and Davies, Neville},
	journal={Journal of Applied Statistics},
	volume={30},
	number={2},
	pages={205--223},
	year={2003},
	publisher={Taylor \& Francis}
}


@article{caiado2006periodogram,
	title={A periodogram-based metric for time series classification},
	author={Caiado, Jorge and Crato, Nuno and Pe{\~n}a, Daniel},
	journal={Computational Statistics \& Data Analysis},
	volume={50},
	number={10},
	pages={2668--2684},
	year={2006},
	publisher={Elsevier}
}

@article{campbell1993trading,
	title={Trading volume and serial correlation in stock returns},
	author={Campbell, John Y and Grossman, Sanford J and Wang, Jiang},
	journal={The Quarterly Journal of Economics},
	volume={108},
	number={4},
	pages={905--939},
	year={1993},
	publisher={MIT Press}
}


@article{campello2007fuzzy,
	title={A fuzzy extension of the Rand index and other related indexes for clustering and classification assessment},
	author={Campello, Ricardo JGB},
	journal={Pattern Recognition Letters},
	volume={28},
	number={7},
	pages={833--841},
	year={2007},
	publisher={Elsevier}
}


@article{cannon1986efficient,
	title={Efficient implementation of the fuzzy c-means clustering algorithms},
	author={Cannon, Robert L and Dave, Jitendra V and Bezdek, James C},
	journal={IEEE transactions on pattern analysis and machine intelligence},
	number={2},
	pages={248--255},
	year={1986},
	publisher={IEEE}
}



@article{caporin2012we,
	title={Do we really need both BEKK and DCC? A tale of two multivariate GARCH models},
	author={Caporin, Massimiliano and McAleer, Michael},
	journal={Journal of Economic Surveys},
	volume={26},
	number={4},
	pages={736--751},
	year={2012},
	publisher={Wiley Online Library}
}


@article{caroni2004detecting,
	title={Detecting an innovative outlier in a set of time series},
	author={Caroni, C and Karioti, V},
	journal={Computational statistics \& data analysis},
	volume={46},
	number={3},
	pages={561--570},
	year={2004},
	publisher={Elsevier}
}

@article{chen2012revisiting,
	title={Revisiting the empirical linkages between stock returns and trading volume},
	author={Chen, Shiu-Sheng},
	journal={Journal of Banking \& Finance},
	volume={36},
	number={6},
	pages={1781--1788},
	year={2012},
	publisher={Elsevier}
}

@inproceedings{cheng2009detection,
	title={Detection and characterization of anomalies in multivariate time series},
	author={Cheng, Haibin and Tan, Pang-Ning and Potter, Christopher and Klooster, Steven},
	booktitle={Proceedings of the 2009 SIAM international conference on data mining},
	pages={413--424},
	year={2009},
	organization={SIAM}
}


@article{chen2013absolute,
	title={Absolute approximation of Tukey depth: Theory and experiments},
	author={Chen, Dan and Morin, Pat and Wagner, Uli},
	journal={Computational Geometry},
	volume={46},
	number={5},
	pages={566--573},
	year={2013},
	publisher={Elsevier}
}


@article{chevallier2012time,
	title={Time-varying correlations in oil, gas and CO2 prices: an application using BEKK, CCC and DCC-MGARCH models},
	author={Chevallier, Julien},
	journal={Applied Economics},
	volume={44},
	number={32},
	pages={4257--4274},
	year={2012},
	publisher={Taylor \& Francis}
}



@inproceedings{cimino2004noise,
	title={On the Noise Distance in Robust Fuzzy C-Means.},
	author={Cimino, Mario GCA and Frosini, Graziano and Lazzerini, Beatrice and Marcelloni, Francesco},
	booktitle={International Conference on Computational Intelligence},
	pages={361--364},
	year={2004}
}


@article{cucina2014outliers,
	title={Outliers detection in multivariate time series using genetic algorithms},
	author={Cucina, Domenico and Di Salvatore, Antonietta and Protopapas, Mattheos K},
	journal={Chemometrics and Intelligent Laboratory Systems},
	volume={132},
	pages={103--110},
	year={2014},
	publisher={Elsevier}
}


@article{cuevas2007robust,
	title={Robust estimation and classification for functional data via projection-based depth notions},
	author={Cuevas, Antonio and Febrero, Manuel and Fraiman, Ricardo},
	journal={Computational Statistics},
	volume={22},
	number={3},
	pages={481--496},
	year={2007},
	publisher={Springer}
}


%D


@article{dave1991characterization,
	title={Characterization and detection of noise in clustering},
	author={Dave, Rajesh N},
	journal={Pattern Recognition Letters},
	volume={12},
	number={11},
	pages={657--664},
	year={1991},
	publisher={Elsevier}
}


@article{dave1997robust,
	title={Robust clustering methods: a unified view},
	author={Dav{\'e}, Rajesh N and Krishnapuram, Raghuram},
	journal={IEEE Transactions on Fuzzy systems},
	volume={5},
	number={2},
	pages={270--293},
	year={1997},
	publisher={IEEE}
}



@inproceedings{dave1997noise,
	title={Noise clustering algorithm revisited},
	author={Dav{\'e}, RN and Sen, Sumit},
	booktitle={1997 Annual Meeting of the North American Fuzzy Information Processing Society-NAFIPS (Cat. No. 97TH8297)},
	pages={199--204},
	year={1997},
	organization={IEEE}
}


@article{dave2002robust,
	title={Robust fuzzy clustering of relational data},
	author={Dav{\'e}, Rajesh N and Sen, Sumit},
	journal={IEEE Transactions on Fuzzy Systems},
	volume={10},
	number={6},
	pages={713--727},
	year={2002},
	publisher={IEEE}
}


@book{davis2007methods,
	title={Methods of numerical integration},
	author={Davis, Philip J and Rabinowitz, Philip},
	year={2007},
	publisher={Courier Corporation}
}


@inproceedings{delgado2012parameters,
	title={Parameters estimation for nonlinear moving average model using Supernova metaheuristic},
	author={Delgado, Eddy Mesa and Cogollo, Myladis R and Vel{\'a}squez, Juan David},
	booktitle={2012 7th Colombian Computing Congress (CCC)},
	pages={1--5},
	year={2012},
	organization={IEEE}
}


@article{dembele2003fuzzy,
	title={Fuzzy C-means method for clustering microarray data},
	author={Dembele, Doulaye and Kastner, Philippe},
	journal={bioinformatics},
	volume={19},
	number={8},
	pages={973--980},
	year={2003},
	publisher={Oxford University Press}
}


@incollection{depayras2018hidden,
	title={The Hidden Face of Nitrogen Oxides Species: From Toxic Effects to Potential Cure?},
	author={Depayras, S{\'e}gol{\`e}ne and Kondakova, Tatiana and Heipieper, Hermann Josef and Feuilloley, Marc GJ and Orange, Nicole and Duclairoir-Poc, C{\'e}cile},
	booktitle={Emerging Pollutants-Some Strategies for the Quality Preservation of Our Environment},
	year={2018},
	publisher={IntechOpen}
}


@inproceedings{ding2004k,
	title={K-means clustering via principal component analysis},
	author={Ding, Chris and He, Xiaofeng},
	booktitle={Proceedings of the twenty-first international conference on Machine learning},
	pages={29},
	year={2004}
}


@article{dias2015clustering,
	title={Clustering financial time series: New insights from an extended hidden Markov model},
	author={Dias, Jos{\'e} G and Vermunt, Jeroen K and Ramos, Sofia},
	journal={European Journal of Operational Research},
	volume={243},
	number={3},
	pages={852--864},
	year={2015},
	publisher={Elsevier}
}


@article{durante2014clustering,
	title={Clustering of financial time series in risky scenarios},
	author={Durante, Fabrizio and Pappad{\`a}, Roberta and Torelli, Nicola},
	journal={Advances in Data Analysis and Classification},
	volume={8},
	number={4},
	pages={359--376},
	year={2014},
	publisher={Springer}
}


@article{d2009autocorrelation,
	title={Autocorrelation-based fuzzy clustering of time series},
	author={D’Urso, Pierpaolo and Maharaj, Elizabeth Ann},
	journal={Fuzzy Sets and Systems},
	volume={160},
	number={24},
	pages={3565--3589},
	year={2009},
	publisher={Elsevier}
}



@article{d2012wavelets,
	title={Wavelets-based clustering of multivariate time series},
	author={D'Urso, Pierpaolo and Maharaj, Elizabeth Ann},
	journal={Fuzzy Sets and Systems},
	volume={193},
	pages={33--61},
	year={2012},
	publisher={Elsevier}
}



@article{d2013noise,
	title={Noise fuzzy clustering of time series by autoregressive metric},
	author={D’Urso, Pierpaolo and De Giovanni, Livia and Massari, Riccardo and Di Lallo, Dario},
	journal={Metron},
	volume={71},
	number={3},
	pages={217--243},
	year={2013},
	publisher={Springer}
}


@article{d2013clustering,
	title={Clustering of financial time series},
	author={D’Urso, Pierpaolo and Cappelli, Carmela and Di Lallo, Dario and Massari, Riccardo},
	journal={Physica A: Statistical Mechanics and its Applications},
	volume={392},
	number={9},
	pages={2114--2129},
	year={2013},
	publisher={Elsevier}
}


@article{d2014wavelet,
	title={Wavelet-based self-organizing maps for classifying multivariate time series},
	author={D'Urso, Pierpaolo and De Giovanni, Livia and Maharaj, Elizabeth Ann and Massari, Riccardo},
	journal={Journal of Chemometrics},
	volume={28},
	number={1},
	pages={28--51},
	year={2014},
	publisher={Wiley Online Library}
}


@article{d2015time,
	title={Time series clustering by a robust autoregressive metric with application to air pollution},
	author={D'Urso, Pierpaolo and De Giovanni, Livia and Massari, Riccardo},
	journal={Chemometrics and Intelligent Laboratory Systems},
	volume={141},
	pages={107--124},
	year={2015},
	publisher={Elsevier}
}


@article{d2017autoregressive,
	title={Autoregressive metric-based trimmed fuzzy clustering with an application to PM10 time series},
	author={D'Urso, Pierpaolo and Massari, Riccardo and Cappelli, Carmela and De Giovanni, Livia},
	journal={Chemometrics and Intelligent Laboratory Systems},
	volume={161},
	pages={15--26},
	year={2017},
	publisher={Elsevier}
}



@article{d2012wavelets,
	title={Wavelets-based clustering of multivariate time series},
	author={D'Urso, Pierpaolo and Maharaj, Elizabeth Ann},
	journal={Fuzzy Sets and Systems},
	volume={193},
	pages={33--61},
	year={2012},
	publisher={Elsevier}
}


@article{d2013clustering,
	title={Clustering of financial time series},
	author={D’Urso, Pierpaolo and Cappelli, Carmela and Di Lallo, Dario and Massari, Riccardo},
	journal={Physica A: Statistical Mechanics and its Applications},
	volume={392},
	number={9},
	pages={2114--2129},
	year={2013},
	publisher={Elsevier}
}


@article{d2014robust,
	title={Robust clustering of imprecise data},
	author={D'Urso, Pierpaolo and De Giovanni, Livia},
	journal={Chemometrics and Intelligent Laboratory Systems},
	volume={136},
	pages={58--80},
	year={2014},
	publisher={Elsevier}
}


@article{d2016garch,
	title={GARCH-based robust clustering of time series},
	author={D'Urso, Pierpaolo and De Giovanni, Livia and Massari, Riccardo},
	journal={Fuzzy Sets and Systems},
	volume={305},
	pages={1--28},
	year={2016},
	publisher={Elsevier}
}




@article{DUrso_De_Giovanni_Maharaj_Massari:2014,
	author = {D'Urso, Pierpaolo and De Giovanni, Livia and Maharaj, Elizabeth Ann and Massari, Riccardo},
	title = {Wavelet-based self-organizing maps for classifying multivariate time series},
	journal = {Journal of Chemometrics},
	volume = {28},
	number = {1},
	pages = {28-51},
	year = {2014}
}

@article{d2018robust,
	title={Robust fuzzy clustering of multivariate time trajectories},
	author={D'Urso, Pierpaolo and De Giovanni, Livia and Massari, Riccardo},
	journal={International Journal of Approximate Reasoning},
	volume={99},
	pages={12--38},
	year={2018},
	publisher={Elsevier}
}



@article{d2005fuzzy,
	title={Fuzzy clustering for data time arrays with inlier and outlier time trajectories},
	author={D'Urso, Pierpaolo},
	journal={IEEE Transactions on Fuzzy Systems},
	volume={13},
	number={5},
	pages={583--604},
	year={2005},
	publisher={IEEE}
}

@article{d2019trimmed,
	title={Trimmed fuzzy clustering of financial time series based on dynamic time warping},
	author={D’Urso, Pierpaolo and De Giovanni, Livia and Massari, Riccardo},
	journal={Annals of operations research},
	pages={1--17},
	year={2019},
	publisher={Springer}
}

%E

@article{efimova2014energy,
	title={Energy markets volatility modelling using GARCH},
	author={Efimova, Olga and Serletis, Apostolos},
	journal={Energy Economics},
	volume={43},
	pages={264--273},
	year={2014},
	publisher={Elsevier}
}

@article{engle1995multivariate,
	title={Multivariate simultaneous generalized ARCH},
	author={Engle, Robert F and Kroner, Kenneth F},
	journal={Econometric theory},
	pages={122--150},
	year={1995},
	publisher={JSTOR}
}


@article{engle2002dynamic,
	title={Dynamic conditional correlation: A simple class of multivariate generalized autoregressive conditional heteroskedasticity models},
	author={Engle, Robert},
	journal={Journal of Business \& Economic Statistics},
	volume={20},
	number={3},
	pages={339--350},
	year={2002},
	publisher={Taylor \& Francis}
}


@article{elsayed1994toxicity,
	title={Toxicity of nitrogen dioxide: an introduction},
	author={Elsayed, Nabil M},
	journal={Toxicology},
	volume={89},
	number={3},
	pages={161--174},
	year={1994},
	publisher={Elsevier}
}


@misc{everitt2011cluster,
	title={Cluster analysis 5th ed},
	author={Everitt, Brian S and Landau, Sabine and Leese, Morven and Stahl, Daniel},
	year={2011},
	publisher={John Wiley}
}

%F


@article{fraiman2001trimmed,
	title={Trimmed means for functional data},
	author={Fraiman, Ricardo and Muniz, Graciela},
	journal={Test},
	volume={10},
	number={2},
	pages={419--440},
	year={2001},
	publisher={Springer}
}


%G

@article{gaitani2010using,
	title={Using principal component and cluster analysis in the heating evaluation of the school building sector},
	author={Gaitani, N and Lehmann, C and Santamouris, M and Mihalakakou, G and Patargias, P},
	journal={Applied Energy},
	volume={87},
	number={6},
	pages={2079--2086},
	year={2010},
	publisher={Elsevier}
}

@article{galeano2006outlier,
	title={Outlier detection in multivariate time series by projection pursuit},
	author={Galeano, Pedro and Pe{\~n}a, Daniel and Tsay, Ruey S},
	journal={Journal of the American Statistical Association},
	volume={101},
	number={474},
	pages={654--669},
	year={2006},
	publisher={Taylor \& Francis}
}

@article{gebka2013causality,
	title={Causality between trading volume and returns: Evidence from quantile regressions},
	author={Gebka, Bartosz and Wohar, Mark E},
	journal={International Review of Economics \& Finance},
	volume={27},
	pages={144--159},
	year={2013},
	publisher={Elsevier}
}


@article{goldberger2000physiobank,
	title={PhysioBank, PhysioToolkit, and PhysioNet: components of a new research resource for complex physiologic signals},
	author={Goldberger, Ary L and Amaral, Luis AN and Glass, Leon and Hausdorff, Jeffrey M and Ivanov, Plamen Ch and Mark, Roger G and Mietus, Joseph E and Moody, George B and Peng, Chung-Kang and Stanley, H Eugene},
	journal={circulation},
	volume={101},
	number={23},
	pages={e215--e220},
	year={2000},
	publisher={Am Heart Assoc}
}

@article{granger1978introduction,
	title={An introduction to bilinear time series models},
	author={Granger, Clive William John and CWJ, GRANGER and AP, ANDERSEN},
	year={1978}
}

@article{granger1993modelling,
	title={Modelling non-linear economic relationships},
	author={Granger, Clive WJ and Terasvirta, Timo and others},
	journal={OUP Catalogue},
	year={1993},
	publisher={Oxford University Press}
}

%H


@article{hair2009multivariate,
	title={Multivariate data analysis},
	author={Hair, Joseph F},
	year={2009}
}

@article{hall1992comparison,
	title={A comparison of neural network and fuzzy clustering techniques in segmenting magnetic resonance images of the brain},
	author={Hall, Lawrence O and Bensaid, Amine M and Clarke, Laurence P and Velthuizen, Robert P and Silbiger, Martin S and Bezdek, James C},
	journal={IEEE transactions on neural networks},
	volume={3},
	number={5},
	pages={672--682},
	year={1992},
	publisher={IEEE}
}

@article{harris2020elastic,
	title={Elastic depths for detecting shape anomalies in functional data},
	author={Harris, Trevor and Tucker, J Derek and Li, Bo and Shand, Lyndsay},
	journal={Technometrics},
	pages={1--11},
	year={2020},
	publisher={Taylor \& Francis}
}

@book{harvey2013dynamic,
	title={Dynamic models for volatility and heavy tails: with applications to financial and economic time series},
	author={Harvey, Andrew C},
	volume={52},
	year={2013},
	publisher={Cambridge University Press}
}

@article{he2018unsupervised,
	title={Unsupervised classification of multivariate time series using VPCA and fuzzy clustering with spatial weighted matrix distance},
	author={He, Hong and Tan, Yonghong},
	journal={IEEE transactions on cybernetics},
	volume={50},
	number={3},
	pages={1096--1105},
	year={2018},
	publisher={IEEE}
}


@article{heidari2013inflation,
	title={Inflation, inflation uncertainty and growth in the Iranian economy: an application of BGARCH-M model with BEKK approach},
	author={Heidari, Hassan and Katircioglu, Salih Turan and Bashiri, Sahar},
	journal={Journal of Business Economics and Management},
	volume={14},
	number={5},
	pages={819--832},
	year={2013},
	publisher={Taylor \& Francis}
}

@article{hoare1962quicksort,
	title={Quicksort},
	author={Hoare, Charles AR},
	journal={The Computer Journal},
	volume={5},
	number={1},
	pages={10--16},
	year={1962},
	publisher={Oxford University Press}
}

@book{hoppner1999fuzzy,
  title={Fuzzy cluster analysis: methods for classification, data analysis and image recognition},
  author={H{\"o}ppner, Frank and Klawonn, Frank and Kruse, Rudolf and Runkler, Thomas},
  year={1999},
  publisher={John Wiley \& Sons}
}

@inproceedings{hyndman2015large,
	title={Large-scale unusual time series detection},
	author={Hyndman, Rob J and Wang, Earo and Laptev, Nikolay},
	booktitle={2015 IEEE international conference on data mining workshop (ICDMW)},
	pages={1616--1619},
	year={2015},
	organization={IEEE}
}


%I

@article{izakian2015fuzzy,
	title={Fuzzy clustering of time series data using dynamic time warping distance},
	author={Izakian, Hesam and Pedrycz, Witold and Jamal, Iqbal},
	journal={Engineering Applications of Artificial Intelligence},
	volume={39},
	pages={235--244},
	year={2015},
	publisher={Elsevier}
}


%K


@inproceedings{kachuee2018ecg,
	title={Ecg heartbeat classification: A deep transferable representation},
	author={Kachuee, Mohammad and Fazeli, Shayan and Sarrafzadeh, Majid},
	booktitle={2018 IEEE International Conference on Healthcare Informatics (ICHI)},
	pages={443--444},
	year={2018},
	organization={IEEE}
}


@article{kakizawa1998discrimination,
	title={Discrimination and clustering for multivariate time series},
	author={Kakizawa, Yoshihide and Shumway, Robert H and Taniguchi, Masanobu},
	journal={Journal of the American Statistical Association},
	volume={93},
	number={441},
	pages={328--340},
	year={1998},
	publisher={Taylor \& Francis Group}
}


@article{karioti2002detecting,
	title={Detecting outlying series in sets of short time series},
	author={Karioti, V and Caroni, C},
	journal={Computational statistics \& data analysis},
	volume={39},
	number={3},
	pages={351--364},
	year={2002},
	publisher={Elsevier}
}


@article{karpoff1987relation,
	title={The relation between price changes and trading volume: A survey},
	author={Karpoff, Jonathan M},
	journal={Journal of Financial and quantitative Analysis},
	pages={109--126},
	year={1987},
	publisher={JSTOR}
}


@phdthesis{khan2015advances,
	title={Advances in applied nonlinear time series modeling},
	author={Khan, Muhammad Yousaf},
	year={2015},
	school={lmu}
}


@article{kou2014evaluation,
	title={Evaluation of clustering algorithms for financial risk analysis using MCDM methods},
	author={Kou, Gang and Peng, Yi and Wang, Guoxun},
	journal={Information Sciences},
	volume={275},
	pages={1--12},
	year={2014},
	publisher={Elsevier}
}




@inproceedings{karakucs2016bayesian,
	title={Bayesian estimation of polynomial moving average models with unknown degree of nonlinearity},
	author={Karaku{\c{s}}, Oktay and Kuruo{\u{g}}lu, Ercan E and Alt{\i}nkaya, Mustafa A},
	booktitle={2016 24th European Signal Processing Conference (EUSIPCO)},
	pages={1543--1547},
	year={2016},
	organization={Ieee}
}




@article{Kley_Volgushev_Dette_Hallin:2016,
	author = "Kley, Tobias and Volgushev, Stanislav and Dette, Holger and Hallin, Marc",
	fjournal = "Bernoulli",
	journal = "Bernoulli",
	month = "08",
	number = "3",
	pages = "1770--1807",
	publisher = "Bernoulli Society for Mathematical Statistics and Probability",
	title = "Quantile spectral processes: Asymptotic analysis and inference",
	volume = "22",
	year = "2016"
}

@article{Koop1996,
	author = {Koop, Gary and Pesaran, M. Hashem and Potter, Simon M.},
	issn = {03044076},
	journal = {Journal of Econometrics},
	keywords = {Impulse response functions,Nonlinear vector autoregressions,Persistence,Threshold autoregressive models},
	number = {1},
	pages = {119--147},
	title = {{Impulse response analysis in nonlinear multivariate models}},
	volume = {74},
	year = {1996}
}

@inproceedings{krishnapuram1999fuzzy,
	title={A fuzzy relative of the k-medoids algorithm with application to web document and snippet clustering},
	author={Krishnapuram, Raghu and Joshi, Anupam and Yi, Liyu},
	booktitle={FUZZ-IEEE'99. 1999 IEEE International Fuzzy Systems. Conference Proceedings (Cat. No. 99CH36315)},
	volume={3},
	pages={1281--1286},
	year={1999},
	organization={IEEE}
}



@article{krishnapuram2001low,
	title={Low-complexity fuzzy relational clustering algorithms for web mining},
	author={Krishnapuram, Raghu and Joshi, Anupam and Nasraoui, Olfa and Yi, Liyu},
	journal={IEEE transactions on Fuzzy Systems},
	volume={9},
	number={4},
	pages={595--607},
	year={2001},
	publisher={IEEE}
}

@article{ku2007application,
	title={On the application of the dynamic conditional correlation model in estimating optimal time-varying hedge ratios},
	author={Ku, Yuan-Hung Hsu and Chen, Ho-Chyuan and Chen, Kuang-hua},
	journal={Applied Economics Letters},
	volume={14},
	number={7},
	pages={503--509},
	year={2007},
	publisher={Taylor \& Francis}
}


@article{kuper2007dynamic,
	title={Dynamic conditional correlation analysis of financial market interdependence: An application to Thailand and Indonesia},
	author={Kuper, Gerard H and others},
	journal={Journal of Asian Economics},
	volume={18},
	number={4},
	pages={670--684},
	year={2007},
	publisher={Elsevier}
}


@article{kwon1998cluster,
	title={Cluster validity index for fuzzy clustering},
	author={Kwon, Soon H},
	journal={Electronics letters},
	volume={34},
	number={22},
	pages={2176--2177},
	year={1998},
	publisher={IET}
}

%L

@article{lafuente2016clustering,
	title={Clustering of time series using quantile autocovariances},
	author={Lafuente-Rego, Borja and Vilar, Jos{\'e} A},
	journal={Advances in Data Analysis and classification},
	volume={10},
	number={3},
	pages={391--415},
	year={2016},
	publisher={Springer}
}


@article{lafuente2018robust,
	title={Robust fuzzy clustering based on quantile autocovariances},
	author={Lafuente-Rego, B and D’Urso, P and Vilar, JA},
	journal={Statistical papers},
	pages={1--56},
	year={2018},
	publisher={Springer}
}



@article{liao2005clustering,
	title={Clustering of time series data—a survey},
	author={Liao, T Warren},
	journal={Pattern recognition},
	volume={38},
	number={11},
	pages={1857--1874},
	year={2005},
	publisher={Elsevier}
}


@article{liu1999multivariate,
	title={Multivariate analysis by data depth: descriptive statistics, graphics and inference,(with discussion and a rejoinder by liu and singh)},
	author={Liu, Regina Y and Parelius, Jesse M and Singh, Kesar and others},
	journal={The annals of statistics},
	volume={27},
	number={3},
	pages={783--858},
	year={1999},
	publisher={Institute of Mathematical Statistics}
}

@article{ljung1993outlier,
	title={On outlier detection in time series},
	author={Ljung, Greta M},
	journal={Journal of the Royal Statistical Society: Series B (Methodological)},
	volume={55},
	number={2},
	pages={559--567},
	year={1993},
	publisher={Wiley Online Library}
}

@article{lopez2009concept,
	title={On the concept of depth for functional data},
	author={L{\'o}pez-Pintado, Sara and Romo, Juan},
	journal={Journal of the American statistical Association},
	volume={104},
	number={486},
	pages={718--734},
	year={2009},
	publisher={Taylor \& Francis}
}

@article{lopez2021quantile,
  title={Quantile cross-spectral density: A novel and effective tool for clustering multivariate time series},
  author={L{\'o}pez-Oriona, {\'A}ngel and Vilar, Jos{\'e} A},
  journal={Expert Systems with Applications},
  volume={185},
  pages={115677},
  year={2021},
  publisher={Elsevier}
}


@article{lu2003nonlinear,
	title={Nonlinear autoregressive and nonlinear autoregressive moving average model parameter estimation by minimizing hypersurface distance},
	author={Lu, Sheng and Chon, Ki H},
	journal={IEEE transactions on signal processing},
	volume={51},
	number={12},
	pages={3020--3026},
	year={2003},
	publisher={IEEE}
}


%M


@article{maharaj1996significance,
	title={A significance test for classifying ARMA models},
	author={Maharaj, Elizabeth Ann},
	journal={Journal of Statistical Computation and Simulation},
	volume={54},
	number={4},
	pages={305--331},
	year={1996},
	publisher={Taylor \& Francis}
}

@article{maharaj1999comparison,
	title={Comparison and classification of stationary multivariate time series},
	author={Maharaj, Elizabeth Ann},
	journal={Pattern Recognition},
	volume={32},
	number={7},
	pages={1129--1138},
	year={1999},
	publisher={Elsevier}
}


@article{maharaj2011fuzzy,
	title={Fuzzy clustering of time series in the frequency domain},
	author={Maharaj, Elizabeth Ann and D’Urso, Pierpaolo},
	journal={Information Sciences},
	volume={181},
	number={7},
	pages={1187--1211},
	year={2011},
	publisher={Elsevier}
}



@article{maharaj2014discriminant,
	title={Discriminant analysis of multivariate time series: Application to diagnosis based on ECG signals},
	author={Maharaj, Elizabeth Ann and Alonso, Andr{\'e}s M},
	journal={Computational Statistics \& Data Analysis},
	volume={70},
	pages={67--87},
	year={2014},
	publisher={Elsevier}
}


@book{maharaj2019time,
	title={Time series clustering and classification},
	author={Maharaj, Elizabeth Ann and D'Urso, Pierpaolo and Caiado, Jorge},
	year={2019},
	publisher={CRC Press}
}


@article{mehlman1987toxicity,
	title={Toxicity and biochemical mechanisms of ozone},
	author={Mehlman, Myron A and Borek, Carmia},
	journal={Environmental research},
	volume={42},
	number={1},
	pages={36--53},
	year={1987},
	publisher={Elsevier}
}


@article{mikosch2003modeling,
	title={Modeling dependence and tails of financial time series},
	author={Mikosch, Thomas},
	journal={Extreme Values in Finance, Telecommunications, and the Environment},
	pages={185--286},
	year={2003}
}


%N

@article{naoui2010dynamic,
	title={A dynamic conditional correlation analysis of financial contagion: the case of the subprime credit crisis},
	author={Naoui, Kamel and Liouane, Naoufel and Brahim, Salem},
	journal={International Journal of Economics and Finance},
	volume={2},
	number={3},
	pages={85--96},
	year={2010}
}

%O


@article{oriona2020,
	author = {L{\'{o}}pez-Oriona, {\'{A}}ngel and Vilar, Jos{\'{e}} A.},
	issn = {18625355},
	journal = {Manuscript submitted 
	for publication},
	title = {{Quantile cross-spectral density: A novel and effective tool for clustering multivariate time series}},
	year = {2020}
}



@article{oriona2021a,
	author = {L{\'{o}}pez-Oriona, {\'{A}}ngel and Vilar, Jos{\'{e}} A.},
	issn = {18625355},
	journal = {Manuscript submitted 
	for publication},
	title = {{F4: An all-purpose tool for multivariate time series classification}},
	year = {2021}
}


@article{oriona2021b,
	author = {L{\'{o}}pez-Oriona, {\'{A}}ngel and Vilar, Jos{\'{e}} A.},
	issn = {18625355},
	journal = {Manuscript submitted 
	for publication},
	title = {{Outlier detection for multivariate time series: a functional data approach}},
	year = {2021}
}



@article{oriona2021c,
	author = {L{\'{o}}pez-Oriona, {\'{A}}ngel and Vilar, Jos{\'{e}} A. and D'Urso, Pierpaolo},
	issn = {18625355},
	journal = {Manuscript submitted 
	for publication},
	title = {{Quantile-based fuzzy clustering of multivariate time series in the frequency domain}},
	year = {2021}
}



%P


@article{pattarin2004clustering,
	title={Clustering financial time series: an application to mutual funds style analysis},
	author={Pattarin, Francesco and Paterlini, Sandra and Minerva, Tommaso},
	journal={Computational Statistics \& Data Analysis},
	volume={47},
	number={2},
	pages={353--372},
	year={2004},
	publisher={Elsevier}
}

@article{pham2010hybrid,
	title={A hybrid of nonlinear autoregressive model with exogenous input and autoregressive moving average model for long-term machine state forecasting},
	author={Pham, Hong Thom and Yang, Bo-Suk and others},
	journal={Expert Systems with Applications},
	volume={37},
	number={4},
	pages={3310--3317},
	year={2010},
	publisher={Elsevier}
}

@article{pereda2005nonlinear,
	title={Nonlinear multivariate analysis of neurophysiological signals},
	author={Pereda, Ernesto and Quiroga, Rodrigo Quian and Bhattacharya, Joydeep},
	journal={Progress in neurobiology},
	volume={77},
	number={1-2},
	pages={1--37},
	year={2005},
	publisher={Elsevier}
}


@article{perron2003searching,
	title={Searching for additive outliers in nonstationary time series},
	author={Perron, Pierre and Rodr{\'\i}guez, Gabriel},
	journal={Journal of Time Series Analysis},
	volume={24},
	number={2},
	pages={193--220},
	year={2003},
	publisher={Wiley Online Library}
}

@article{piccolo1990distance,
	title={A distance measure for classifying ARIMA models},
	author={Piccolo, Domenico},
	journal={Journal of Time Series Analysis},
	volume={11},
	number={2},
	pages={153--164},
	year={1990},
	publisher={Wiley Online Library}
}


%R


@book{rachev2003handbook,
	title={Handbook of Heavy Tailed Distributions in Finance: Handbooks in Finance, Book 1},
	author={Rachev, Svetlozar Todorov},
	year={2003},
	publisher={Elsevier}
}


@article{rahman2012oil,
	title={Oil price uncertainty and the Canadian economy: Evidence from a VARMA, GARCH-in-Mean, asymmetric BEKK model},
	author={Rahman, Sajjadur and Serletis, Apostolos},
	journal={Energy Economics},
	volume={34},
	number={2},
	pages={603--610},
	year={2012},
	publisher={Elsevier}
}

@incollection{raychaudhuri1999principal,
	title={Principal components analysis to summarize microarray experiments: application to sporulation time series},
	author={Raychaudhuri, Soumya and Stuart, Joshua M and Altman, Russ B},
	booktitle={Biocomputing 2000},
	pages={455--466},
	year={1999},
	publisher={World Scientific}
}

@article{rebbapragada2009finding,
	title={Finding anomalous periodic time series},
	author={Rebbapragada, Umaa and Protopapas, Pavlos and Brodley, Carla E and Alcock, Charles},
	journal={Machine learning},
	volume={74},
	number={3},
	pages={281--313},
	year={2009},
	publisher={Springer}
}


@article{remya2016classification,
	title={Classification of myocardial infarction using multi resolution wavelet analysis of ECG},
	author={Remya, RS and Indiradevi, KP and Babu, KK Anish},
	journal={Procedia Technology},
	volume={24},
	pages={949--956},
	year={2016},
	publisher={Elsevier}
}


@inproceedings{rivera2017robust,
	title={Robust clustering for time series using spectral densities and functional data analysis},
	author={Rivera-Garc{\'\i}a, Diego and Garc{\'\i}a-Escudero, Luis Angel and Mayo-Iscar, Agust{\'\i}n and Ortega, Joaqu{\'\i}n},
	booktitle={International Work-Conference on Artificial Neural Networks},
	pages={142--153},
	year={2017},
	organization={Springer}
}

%S


@article{sadhukhan2018automated,
	title={Automated identification of myocardial infarction using harmonic phase distribution pattern of ECG data},
	author={Sadhukhan, Deboleena and Pal, Saurabh and Mitra, Madhuchhanda},
	journal={IEEE Transactions on Instrumentation and Measurement},
	volume={67},
	number={10},
	pages={2303--2313},
	year={2018},
	publisher={IEEE}
}


@article{schmitt2013non,
	title={Non-stationarity in financial time series: Generic features and tail behavior},
	author={Schmitt, Thilo A and Chetalova, Desislava and Sch{\"a}fer, Rudi and Guhr, Thomas},
	journal={EPL (Europhysics Letters)},
	volume={103},
	number={5},
	pages={58003},
	year={2013},
	publisher={IOP Publishing}
}


@article{schmitt2013non,
	title={Non-stationarity in financial time series: Generic features and tail behavior},
	author={Schmitt, Thilo A and Chetalova, Desislava and Sch{\"a}fer, Rudi and Guhr, Thomas},
	journal={EPL (Europhysics Letters)},
	volume={103},
	number={5},
	pages={58003},
	year={2013},
	publisher={IOP Publishing}
}


@book{shumway2000time,
	title={Time series analysis and its applications},
	author={Shumway, Robert H and Stoffer, David S and Stoffer, David S},
	volume={3},
	year={2000},
	publisher={Springer}
}




%T

@article{takeuchi2006unifying,
	title={A unifying framework for detecting outliers and change points from time series},
	author={Takeuchi, Jun-ichi and Yamanishi, Kenji},
	journal={IEEE transactions on Knowledge and Data Engineering},
	volume={18},
	number={4},
	pages={482--492},
	year={2006},
	publisher={IEEE}
}

@inproceedings{tang2005improved,
	title={Improved validation index for fuzzy clustering},
	author={Tang, Yuangang and Sun, Fuchun and Sun, Zengqi},
	booktitle={Proceedings of the 2005, American Control Conference, 2005.},
	pages={1120--1125},
	year={2005},
	organization={IEEE}
}

@article{tsay2000outliers,
	title={Outliers in multivariate time series},
	author={Tsay, Ruey S and Pena, Daniel and Pankratz, Alan E},
	journal={Biometrika},
	volume={87},
	number={4},
	pages={789--804},
	year={2000},
	publisher={Oxford University Press}
}

@incollection{tong2009threshold,
	title={Threshold autoregression, limit cycles and cyclical data},
	author={Tong, Howell and Lim, Keng S},
	booktitle={Exploration Of A Nonlinear World: An Appreciation of Howell Tong's Contributions to Statistics},
	pages={9--56},
	year={2009},
	publisher={World Scientific}
}

@incollection{tong2009threshold,
	title={Threshold autoregression, limit cycles and cyclical data},
	author={Tong, Howell and Lim, Keng S},
	booktitle={Exploration Of A Nonlinear World: An Appreciation of Howell Tong's Contributions to Statistics},
	pages={9--56},
	year={2009},
	publisher={World Scientific}
}

@incollection{tong2009threshold,
	title={Threshold autoregression, limit cycles and cyclical data},
	author={Tong, Howell and Lim, Keng S},
	booktitle={Exploration Of A Nonlinear World: An Appreciation of Howell Tong's Contributions to Statistics},
	pages={9--56},
	year={2009},
	publisher={World Scientific}
}

@article{tsay2000outliers,
	title={Outliers in multivariate time series},
	author={Tsay, Ruey S and Pena, Daniel and Pankratz, Alan E},
	journal={Biometrika},
	volume={87},
	number={4},
	pages={789--804},
	year={2000},
	publisher={Oxford University Press}
}


@article{tsay1988outliers,
	title={Outliers, level shifts, and variance changes in time series},
	author={Tsay, Ruey S},
	journal={Journal of forecasting},
	volume={7},
	number={1},
	pages={1--20},
	year={1988},
	publisher={Wiley Online Library}
}

%V

@article{vilar2018quantile,
	title={Quantile autocovariances: a powerful tool for hard and soft partitional clustering of time series},
	author={Vilar, Jos{\'e} A and Lafuente-Rego, Borja and D'Urso, Pierpaolo},
	journal={Fuzzy Sets and Systems},
	volume={340},
	pages={38--72},
	year={2018},
	publisher={Elsevier}
}

%W


@inproceedings{wang2007structure,
	title={Structure-based statistical features and multivariate time series clustering},
	author={Wang, Xiaozhe and Wirth, Anthony and Wang, Liang},
	booktitle={Seventh IEEE International Conference on Data Mining (ICDM 2007)},
	pages={351--360},
	year={2007},
	organization={IEEE}
}


@article{weise1999asymmetric,
	title={The asymmetric effects of monetary policy: A nonlinear vector autoregression approach},
	author={Weise, Charles L},
	journal={Journal of Money, Credit and Banking},
	pages={85--108},
	year={1999},
	publisher={JSTOR}
}


@inproceedings{weng2006outlier,
	title={Outlier mining for multivariate time series based on local sparsity coefficient},
	author={Weng, Xiaoqing and Shen, Junyi},
	booktitle={2006 6th World Congress on Intelligent Control and Automation},
	volume={2},
	pages={5957--5961},
	year={2006},
	organization={IEEE}
}


@article{weng2008detecting,
	title={Detecting outlier samples in multivariate time series dataset},
	author={Weng, Xiaoqing and Shen, Junyi},
	journal={Knowledge-based systems},
	volume={21},
	number={8},
	pages={807--812},
	year={2008},
	publisher={Elsevier}
}


@article{wu2002alternative,
	title={Alternative c-means clustering algorithms},
	author={Wu, Kuo-Lung and Yang, Miin-Shen},
	journal={Pattern recognition},
	volume={35},
	number={10},
	pages={2267--2278},
	year={2002},
	publisher={Elsevier}
}


@inproceedings{wu2013dynamic,
	title={Dynamic covariance models for multivariate financial time series},
	author={Wu, Yue and Hern{\'a}ndez-Lobato, Jos{\'e} Miguel and Zoubin, Ghahramani},
	booktitle={International Conference on Machine Learning},
	pages={558--566},
	year={2013},
	organization={PMLR}
}

%X

@article{xie1991validity,
	title={A validity measure for fuzzy clustering},
	author={Xie, Xuanli Lisa and Beni, Gerardo},
	journal={IEEE Transactions on pattern analysis and machine intelligence},
	volume={13},
	number={8},
	pages={841--847},
	year={1991}
}


@article{xue2011using,
	title={Using principal components analysis (PCA) with cluster analysis to study the organic geochemistry of sinking particles in the ocean},
	author={Xue, Jianhong and Lee, Cindy and Wakeham, Stuart G and Armstrong, Robert A},
	journal={Organic Geochemistry},
	volume={42},
	number={4},
	pages={356--367},
	year={2011},
	publisher={Elsevier}
}

%Y 



@inproceedings{yamanishi2002unifying,
	title={A unifying framework for detecting outliers and change points from non-stationary time series data},
	author={Yamanishi, Kenji and Takeuchi, Jun-ichi},
	booktitle={Proceedings of the eighth ACM SIGKDD international conference on Knowledge discovery and data mining},
	pages={676--681},
	year={2002}
}

@inproceedings{yang2004pca,
	title={A PCA-based similarity measure for multivariate time series},
	author={Yang, Kiyoung and Shahabi, Cyrus},
	booktitle={Proceedings of the 2nd ACM international workshop on Multimedia databases},
	pages={65--74},
	year={2004}
}



@article{yassin2016binary,
	title={Binary particle swarm optimization structure selection of nonlinear autoregressive moving average with exogenous inputs (NARMAX) model of a flexible robot arm},
	author={Yassin, Ihsan Mohd and Zabidi, Azlee and Amin Megat Ali, Megat Syahirul and Md Tahir, Nooritawati and Zainol Abidin, Husna and Rizman, Zairi Ismael},
	journal={International Journal on Advanced Science, Engineering and Information Technology},
	volume={6},
	number={5},
	pages={630--637},
	year={2016}
}




%Z

@article{Zhang2001,
	author = {Zhang, G. Peter and Patuwo, B. Eddy and Hu, Michael Y.},
	issn = {03050548},
	journal = {Computers and Operations Research},
	keywords = {Artificial neural networks,Forecasting,Nonlinear time series,Simulation},
	number = {4},
	pages = {381--396},
	title = {{A simulation study of artificial neural networks for nonlinear time-series forecasting}},
	volume = {28},
	year = {2001}
}


@article{zhou2014fuzziness,
	title={Fuzziness parameter selection in fuzzy c-means: the perspective of cluster validation},
	author={Zhou, KaiLe and Fu, Chao and Yang, ShanLin},
	journal={Science China Information Sciences},
	volume={57},
	number={11},
	pages={1--8},
	year={2014},
	publisher={Springer}
}









%A


@article{abraham1989outlier,
	title={Outlier detection and time series modeling},
	author={Abraham, Bovas and Chuang, Alice},
	journal={Technometrics},
	volume={31},
	number={2},
	pages={241--248},
	year={1989},
	publisher={Taylor \& Francis}
}


@inproceedings{agyemang2004lsc,
	title={Lsc-mine: Algorithm for mining local outliers},
	author={Agyemang, Malik and Ezeife, Christie I},
	booktitle={Proceedings of the 15th Information Resource Management Association (IRMA) International Conference, New Orleans},
	volume={1},
	pages={5--8},
	year={2004},
	organization={Citeseer}
}


@article{andersson2008does,
	title={Why does the correlation between stock and bond returns vary over time?},
	author={Andersson, Magnus and Krylova, Elizaveta and V{\"a}h{\"a}maa, Sami},
	journal={Applied Financial Economics},
	volume={18},
	number={2},
	pages={139--151},
	year={2008},
	publisher={Taylor \& Francis}
}


@article{arabie1981overlapping,
	title={Overlapping clustering: A new method for product positioning},
	author={Arabie, Phipps and Carroll, J Douglas and DeSarbo, Wayne and Wind, Jerry},
	journal={Journal of Marketing Research},
	volume={18},
	number={3},
	pages={310--317},
	year={1981},
	publisher={SAGE Publications Sage CA: Los Angeles, CA}
}



@inproceedings{awwad2008nonlinear,
	title={Nonlinear autoregressive moving average (NARMA-L2) controller for advanced ac motor control},
	author={Awwad, A and Abu-Rub, H and Toliyat, HA},
	booktitle={2008 34th Annual Conference of IEEE Industrial Electronics},
	pages={1287--1292},
	year={2008},
	organization={IEEE}
}

%B





@inproceedings{banerjee2010ecg,
	title={ECG feature extraction and classification of anteroseptal myocardial infarction and normal subjects using discrete wavelet transform},
	author={Banerjee, Swati and Mitra, Madhuchhanda},
	booktitle={2010 International Conference on Systems in Medicine and Biology},
	pages={55--60},
	year={2010},
	organization={IEEE}
}


@article{banerjee2013application,
	title={Application of cross wavelet transform for ECG pattern analysis and classification},
	author={Banerjee, Swati and Mitra, Madhuchhanda},
	journal={IEEE transactions on instrumentation and measurement},
	volume={63},
	number={2},
	pages={326--333},
	year={2013},
	publisher={IEEE}
}


@article{baragona2007outliers,
	title={Outliers detection in multivariate time series by independent component analysis},
	author={Baragona, Roberto and Battaglia, Francesco},
	journal={Neural computation},
	volume={19},
	number={7},
	pages={1962--1984},
	year={2007},
	publisher={MIT Press}
}


@article{Barunik_Kley:2019,
	author = {Baruník, Jozef and Kley, Tobias},
	title = "{Quantile coherency: A general measure for dependence between cyclical economic variables}",
	journal = {The Econometrics Journal},
	volume = {22},
	number = {2},
	pages = {131-152},
	year = {2019},
}

@article{bastos2014clustering,
	title={Clustering financial time series with variance ratio statistics},
	author={Bastos, Jo{\~a}o A and Caiado, Jorge},
	journal={Quantitative Finance},
	volume={14},
	number={12},
	pages={2121--2133},
	year={2014},
	publisher={Taylor \& Francis}
}

@article{basu2007automatic,
	title={Automatic outlier detection for time series: an application to sensor data},
	author={Basu, Sabyasachi and Meckesheimer, Martin},
	journal={Knowledge and Information Systems},
	volume={11},
	number={2},
	pages={137--154},
	year={2007},
	publisher={Springer}
}


@article{bauwens2006multivariate,
	title={Multivariate GARCH models: a survey},
	author={Bauwens, Luc and Laurent, S{\'e}bastien and Rombouts, Jeroen VK},
	journal={Journal of applied econometrics},
	volume={21},
	number={1},
	pages={79--109},
	year={2006},
	publisher={Wiley Online Library}
}


@article{battaglia2005outlier,
	title={Outlier detection and estimation in nonlinear time series},
	author={Battaglia, Francesco and Orfei, Lia},
	journal={Journal of Time Series Analysis},
	volume={26},
	number={1},
	pages={107--121},
	year={2005},
	publisher={Wiley Online Library}
}


@article{beggel2019time,
	title={Time series anomaly detection based on shapelet learning},
	author={Beggel, Laura and Kausler, Bernhard X and Schiegg, Martin and Pfeiffer, Michael and Bischl, Bernd},
	journal={Computational Statistics},
	volume={34},
	number={3},
	pages={945--976},
	year={2019},
	publisher={Springer}
}


@incollection{ben2003detecting,
	title={Detecting stable clusters using principal component analysis},
	author={Ben-Hur, Asa and Guyon, Isabelle},
	booktitle={Functional genomics},
	pages={159--182},
	year={2003},
	publisher={Springer}
}


@article{benkabou2018unsupervised,
	title={Unsupervised outlier detection for time series by entropy and dynamic time warping},
	author={Benkabou, Seif-Eddine and Benabdeslem, Khalid and Canitia, Bruno},
	journal={Knowledge and Information Systems},
	volume={54},
	number={2},
	pages={463--486},
	year={2018},
	publisher={Springer}
}


@article{bernardi2017multiple,
	title={Multiple risk measures for multivariate dynamic heavy--tailed models},
	author={Bernardi, Mauro and Maruotti, Antonello and Petrella, Lea},
	journal={Journal of Empirical Finance},
	volume={43},
	pages={1--32},
	year={2017},
	publisher={Elsevier}
}


@article{bensaid1996validity,
	title={Validity-guided (re) clustering with applications to image segmentation},
	author={Bensaid, Amine M and Hall, Lawrence O and Bezdek, James C and Clarke, Laurence P and Silbiger, Martin L and Arrington, John A and Murtagh, Reed F},
	journal={IEEE Transactions on fuzzy systems},
	volume={4},
	number={2},
	pages={112--123},
	year={1996},
	publisher={IEEE}
}
@article{bensaid1996validity,
	title={Validity-guided (re) clustering with applications to image segmentation},
	author={Bensaid, Amine M and Hall, Lawrence O and Bezdek, James C and Clarke, Laurence P and Silbiger, Martin L and Arrington, John A and Murtagh, Reed F},
	journal={IEEE Transactions on fuzzy systems},
	volume={4},
	number={2},
	pages={112--123},
	year={1996},
	publisher={IEEE}
}


@book{bezdek2013pattern,
	title={Pattern recognition with fuzzy objective function algorithms},
	author={Bezdek, James C},
	year={2013},
	publisher={Springer Science \& Business Media}
}

@article{blazquez2020review,
	title={A review on outlier/anomaly detection in time series data},
	author={Bl{\'a}zquez-Garc{\'\i}a, Ane and Conde, Angel and Mori, Usue and Lozano, Jose A},
	journal={arXiv preprint arXiv:2002.04236},
	year={2020}
}


@article{bollerslev1986generalized,
	title={Generalized autoregressive conditional heteroskedasticity},
	author={Bollerslev, Tim},
	journal={Journal of econometrics},
	volume={31},
	number={3},
	pages={307--327},
	year={1986},
	publisher={Elsevier}
}


@book{box2015time,
	title={Time series analysis: forecasting and control},
	author={Box, George EP and Jenkins, Gwilym M and Reinsel, Gregory C and Ljung, Greta M},
	year={2015},
	publisher={John Wiley \& Sons}
}



@inproceedings{boynton2013application,
	title={Application of nonlinear autoregressive moving average exogenous input models to geospace: advances in understanding and space weather forecasts},
	author={Boynton, RJ and Balikhin, MA and Billings, SA and Amariutei, OA},
	booktitle={Annales Geophysicae},
	volume={31},
	number={9},
	pages={1579--1589},
	year={2013},
	organization={Copernicus GmbH}
}


@incollection{bradley2003financial,
	title={Financial risk and heavy tails},
	author={Bradley, Brendan O and Taqqu, Murad S},
	booktitle={Handbook of heavy tailed distributions in finance},
	pages={35--103},
	year={2003},
	publisher={Elsevier}
}


@article{brigham1967fast,
	title={The fast Fourier transform},
	author={Brigham, E Oran and Morrow, RE},
	journal={IEEE spectrum},
	volume={4},
	number={12},
	pages={63--70},
	year={1967},
	publisher={IEEE}
}

%C


@article{cai2003simple,
	title={A simple diagnostic method of outlier detection for stationary Gaussian time series},
	author={Cai, Yuzhi and Davies, Neville},
	journal={Journal of Applied Statistics},
	volume={30},
	number={2},
	pages={205--223},
	year={2003},
	publisher={Taylor \& Francis}
}

@article{campbell1993trading,
	title={Trading volume and serial correlation in stock returns},
	author={Campbell, John Y and Grossman, Sanford J and Wang, Jiang},
	journal={The Quarterly Journal of Economics},
	volume={108},
	number={4},
	pages={905--939},
	year={1993},
	publisher={MIT Press}
}


@article{campello2007fuzzy,
	title={A fuzzy extension of the Rand index and other related indexes for clustering and classification assessment},
	author={Campello, Ricardo JGB},
	journal={Pattern Recognition Letters},
	volume={28},
	number={7},
	pages={833--841},
	year={2007},
	publisher={Elsevier}
}


@article{cannon1986efficient,
	title={Efficient implementation of the fuzzy c-means clustering algorithms},
	author={Cannon, Robert L and Dave, Jitendra V and Bezdek, James C},
	journal={IEEE transactions on pattern analysis and machine intelligence},
	number={2},
	pages={248--255},
	year={1986},
	publisher={IEEE}
}



@article{caroni2004detecting,
	title={Detecting an innovative outlier in a set of time series},
	author={Caroni, C and Karioti, V},
	journal={Computational statistics \& data analysis},
	volume={46},
	number={3},
	pages={561--570},
	year={2004},
	publisher={Elsevier}
}

@article{chen2012revisiting,
	title={Revisiting the empirical linkages between stock returns and trading volume},
	author={Chen, Shiu-Sheng},
	journal={Journal of Banking \& Finance},
	volume={36},
	number={6},
	pages={1781--1788},
	year={2012},
	publisher={Elsevier}
}

@inproceedings{cheng2009detection,
	title={Detection and characterization of anomalies in multivariate time series},
	author={Cheng, Haibin and Tan, Pang-Ning and Potter, Christopher and Klooster, Steven},
	booktitle={Proceedings of the 2009 SIAM international conference on data mining},
	pages={413--424},
	year={2009},
	organization={SIAM}
}


@article{chen2013absolute,
	title={Absolute approximation of Tukey depth: Theory and experiments},
	author={Chen, Dan and Morin, Pat and Wagner, Uli},
	journal={Computational Geometry},
	volume={46},
	number={5},
	pages={566--573},
	year={2013},
	publisher={Elsevier}
}


@article{coppi2006fuzzy,
	title={Fuzzy unsupervised classification of multivariate time trajectories with the Shannon entropy regularization},
	author={Coppi, Renato and D’Urso, Pierpaolo},
	journal={Computational statistics \& data analysis},
	volume={50},
	number={6},
	pages={1452--1477},
	year={2006},
	publisher={Elsevier}
}


@article{cucina2014outliers,
	title={Outliers detection in multivariate time series using genetic algorithms},
	author={Cucina, Domenico and Di Salvatore, Antonietta and Protopapas, Mattheos K},
	journal={Chemometrics and Intelligent Laboratory Systems},
	volume={132},
	pages={103--110},
	year={2014},
	publisher={Elsevier}
}


@article{cuevas2007robust,
	title={Robust estimation and classification for functional data via projection-based depth notions},
	author={Cuevas, Antonio and Febrero, Manuel and Fraiman, Ricardo},
	journal={Computational Statistics},
	volume={22},
	number={3},
	pages={481--496},
	year={2007},
	publisher={Springer}
}


%D


@book{davis2007methods,
	title={Methods of numerical integration},
	author={Davis, Philip J and Rabinowitz, Philip},
	year={2007},
	publisher={Courier Corporation}
}


@inproceedings{delgado2012parameters,
	title={Parameters estimation for nonlinear moving average model using Supernova metaheuristic},
	author={Delgado, Eddy Mesa and Cogollo, Myladis R and Vel{\'a}squez, Juan David},
	booktitle={2012 7th Colombian Computing Congress (CCC)},
	pages={1--5},
	year={2012},
	organization={IEEE}
}


@incollection{depayras2018hidden,
	title={The Hidden Face of Nitrogen Oxides Species: From Toxic Effects to Potential Cure?},
	author={Depayras, S{\'e}gol{\`e}ne and Kondakova, Tatiana and Heipieper, Hermann Josef and Feuilloley, Marc GJ and Orange, Nicole and Duclairoir-Poc, C{\'e}cile},
	booktitle={Emerging Pollutants-Some Strategies for the Quality Preservation of Our Environment},
	year={2018},
	publisher={IntechOpen}
}



@article{Dette_Hallin_Kley_Volgushev:2015,
	author = "Dette, Holger and Hallin, Marc and Kley, Tobias and Volgushev, Stanislav",
	fjournal = "Bernoulli",
	journal = "Bernoulli",
	month = "05",
	number = "2",
	pages = "781--831",
	publisher = "Bernoulli Society for Mathematical Statistics and Probability",
	title = "Of copulas, quantiles, ranks and spectra: An $L_{1}$-approach to spectral analysis",
	volume = "21",
	year = "2015"
}



@article{dias2015clustering,
	title={Clustering financial time series: New insights from an extended hidden Markov model},
	author={Dias, Jos{\'e} G and Vermunt, Jeroen K and Ramos, Sofia},
	journal={European Journal of Operational Research},
	volume={243},
	number={3},
	pages={852--864},
	year={2015},
	publisher={Elsevier}
}

@inproceedings{ding2004k,
	title={K-means clustering via principal component analysis},
	author={Ding, Chris and He, Xiaofeng},
	booktitle={Proceedings of the twenty-first international conference on Machine learning},
	pages={29},
	year={2004}
}

@article{disegna2017copula,
	title={Copula-based fuzzy clustering of spatial time series},
	author={Disegna, Marta and D’Urso, Pierpaolo and Durante, Fabrizio},
	journal={Spatial Statistics},
	volume={21},
	pages={209--225},
	year={2017},
	publisher={Elsevier}
}




@article{durante2014clustering,
	title={Clustering of financial time series in risky scenarios},
	author={Durante, Fabrizio and Pappad{\`a}, Roberta and Torelli, Nicola},
	journal={Advances in Data Analysis and Classification},
	volume={8},
	number={4},
	pages={359--376},
	year={2014},
	publisher={Springer}
}

@article{d2017fuzzy,
	title={Fuzzy clustering of time series using extremes},
	author={D'Urso, Pierpaolo and Maharaj, Elizabeth A and Alonso, Andr{\'e}s M},
	journal={Fuzzy Sets and Systems},
	volume={318},
	pages={56--79},
	year={2017},
	publisher={Elsevier}
}

@article{d2013clustering,
	title={Clustering of financial time series},
	author={D’Urso, Pierpaolo and Cappelli, Carmela and Di Lallo, Dario and Massari, Riccardo},
	journal={Physica A: Statistical Mechanics and its Applications},
	volume={392},
	number={9},
	pages={2114--2129},
	year={2013},
	publisher={Elsevier}
}


@article{d2012wavelets,
	title={Wavelets-based clustering of multivariate time series},
	author={D'Urso, Pierpaolo and Maharaj, Elizabeth Ann},
	journal={Fuzzy Sets and Systems},
	volume={193},
	pages={33--61},
	year={2012},
	publisher={Elsevier}
}

@article{d2009autocorrelation,
	title={Autocorrelation-based fuzzy clustering of time series},
	author={D’Urso, Pierpaolo and Maharaj, Elizabeth Ann},
	journal={Fuzzy Sets and Systems},
	volume={160},
	number={24},
	pages={3565--3589},
	year={2009},
	publisher={Elsevier}
}


%E


@article{2002dynamic,
	title={Dynamic conditional correlation: A simple class of multivariate generalized autoregressive conditional heteroskedasticity models},
	author={Engle, Robert},
	journal={Journal of Business \& Economic Statistics},
	volume={20},
	number={3},
	pages={339--350},
	year={2002},
	publisher={Taylor \& Francis}
}


@article{elsayed1994toxicity,
	title={Toxicity of nitrogen dioxide: an introduction},
	author={Elsayed, Nabil M},
	journal={Toxicology},
	volume={89},
	number={3},
	pages={161--174},
	year={1994},
	publisher={Elsevier}
}


@misc{everitt2011cluster,
	title={Cluster analysis 5th ed},
	author={Everitt, Brian S and Landau, Sabine and Leese, Morven and Stahl, Daniel},
	year={2011},
	publisher={John Wiley}
}

%F


@article{fraiman2001trimmed,
	title={Trimmed means for functional data},
	author={Fraiman, Ricardo and Muniz, Graciela},
	journal={Test},
	volume={10},
	number={2},
	pages={419--440},
	year={2001},
	publisher={Springer}
}


%G

@article{gaitani2010using,
	title={Using principal component and cluster analysis in the heating evaluation of the school building sector},
	author={Gaitani, N and Lehmann, C and Santamouris, M and Mihalakakou, G and Patargias, P},
	journal={Applied Energy},
	volume={87},
	number={6},
	pages={2079--2086},
	year={2010},
	publisher={Elsevier}
}

@article{galeano2006outlier,
	title={Outlier detection in multivariate time series by projection pursuit},
	author={Galeano, Pedro and Pe{\~n}a, Daniel and Tsay, Ruey S},
	journal={Journal of the American Statistical Association},
	volume={101},
	number={474},
	pages={654--669},
	year={2006},
	publisher={Taylor \& Francis}
}

@article{gebka2013causality,
	title={Causality between trading volume and returns: Evidence from quantile regressions},
	author={Gebka, Bartosz and Wohar, Mark E},
	journal={International Review of Economics \& Finance},
	volume={27},
	pages={144--159},
	year={2013},
	publisher={Elsevier}
}


@article{goldberger2000physiobank,
	title={PhysioBank, PhysioToolkit, and PhysioNet: components of a new research resource for complex physiologic signals},
	author={Goldberger, Ary L and Amaral, Luis AN and Glass, Leon and Hausdorff, Jeffrey M and Ivanov, Plamen Ch and Mark, Roger G and Mietus, Joseph E and Moody, George B and Peng, Chung-Kang and Stanley, H Eugene},
	journal={circulation},
	volume={101},
	number={23},
	pages={e215--e220},
	year={2000},
	publisher={Am Heart Assoc}
}

@article{granger1978introduction,
	title={An introduction to bilinear time series models},
	author={Granger, Clive William John and CWJ, GRANGER and AP, ANDERSEN},
	year={1978}
}

@article{granger1993modelling,
	title={Modelling non-linear economic relationships},
	author={Granger, Clive WJ and Terasvirta, Timo and others},
	journal={OUP Catalogue},
	year={1993},
	publisher={Oxford University Press}
}

%H


@article{hair2009multivariate,
	title={Multivariate data analysis},
	author={Hair, Joseph F},
	year={2009}
}

@article{hall1992comparison,
	title={A comparison of neural network and fuzzy clustering techniques in segmenting magnetic resonance images of the brain},
	author={Hall, Lawrence O and Bensaid, Amine M and Clarke, Laurence P and Velthuizen, Robert P and Silbiger, Martin S and Bezdek, James C},
	journal={IEEE transactions on neural networks},
	volume={3},
	number={5},
	pages={672--682},
	year={1992},
	publisher={IEEE}
}

@article{harris2020elastic,
	title={Elastic depths for detecting shape anomalies in functional data},
	author={Harris, Trevor and Tucker, J Derek and Li, Bo and Shand, Lyndsay},
	journal={Technometrics},
	pages={1--11},
	year={2020},
	publisher={Taylor \& Francis}
}

@book{harvey2013dynamic,
	title={Dynamic models for volatility and heavy tails: with applications to financial and economic time series},
	author={Harvey, Andrew C},
	volume={52},
	year={2013},
	publisher={Cambridge University Press}
}

@article{he2018unsupervised,
	title={Unsupervised classification of multivariate time series using VPCA and fuzzy clustering with spatial weighted matrix distance},
	author={He, Hong and Tan, Yonghong},
	journal={IEEE transactions on cybernetics},
	volume={50},
	number={3},
	pages={1096--1105},
	year={2018},
	publisher={IEEE}
}

@article{hoare1962quicksort,
	title={Quicksort},
	author={Hoare, Charles AR},
	journal={The Computer Journal},
	volume={5},
	number={1},
	pages={10--16},
	year={1962},
	publisher={Oxford University Press}
}

@book{hoppner1999fuzzy,
	title={Fuzzy cluster analysis: methods for classification, data analysis and image recognition},
	author={H{\"o}ppner, Frank and Klawonn, Frank and Kruse, Rudolf and Runkler, Thomas},
	year={1999},
	publisher={John Wiley \& Sons}
}

@inproceedings{hyndman2015large,
	title={Large-scale unusual time series detection},
	author={Hyndman, Rob J and Wang, Earo and Laptev, Nikolay},
	booktitle={2015 IEEE international conference on data mining workshop (ICDMW)},
	pages={1616--1619},
	year={2015},
	organization={IEEE}
}


%I


@article{izakian2015fuzzy,
	title={Fuzzy clustering of time series data using dynamic time warping distance},
	author={Izakian, Hesam and Pedrycz, Witold and Jamal, Iqbal},
	journal={Engineering Applications of Artificial Intelligence},
	volume={39},
	pages={235--244},
	year={2015},
	publisher={Elsevier}
}


%K


@inproceedings{kachuee2018ecg,
	title={Ecg heartbeat classification: A deep transferable representation},
	author={Kachuee, Mohammad and Fazeli, Shayan and Sarrafzadeh, Majid},
	booktitle={2018 IEEE International Conference on Healthcare Informatics (ICHI)},
	pages={443--444},
	year={2018},
	organization={IEEE}
}


@article{karioti2002detecting,
	title={Detecting outlying series in sets of short time series},
	author={Karioti, V and Caroni, C},
	journal={Computational statistics \& data analysis},
	volume={39},
	number={3},
	pages={351--364},
	year={2002},
	publisher={Elsevier}
}


@article{karpoff1987relation,
	title={The relation between price changes and trading volume: A survey},
	author={Karpoff, Jonathan M},
	journal={Journal of Financial and quantitative Analysis},
	pages={109--126},
	year={1987},
	publisher={JSTOR}
}


@phdthesis{khan2015advances,
	title={Advances in applied nonlinear time series modeling},
	author={Khan, Muhammad Yousaf},
	year={2015},
	school={lmu}
}


@article{Kley_Volgushev_Dette_Hallin:2016,
	author = "Kley, Tobias and Volgushev, Stanislav and Dette, Holger and Hallin, Marc",
	fjournal = "Bernoulli",
	journal = "Bernoulli",
	month = "08",
	number = "3",
	pages = "1770--1807",
	publisher = "Bernoulli Society for Mathematical Statistics and Probability",
	title = "Quantile spectral processes: Asymptotic analysis and inference",
	volume = "22",
	year = "2016"
}



@Article{Kley_quantspec,
	title = {Quantile-Based Spectral Analysis in an Object-Oriented
	Framework and a Reference Implementation in \proglang{R}: The \pkg{quantspec} Package},
	author = {Tobias Kley},
	journal = {Journal of Statistical Software},
	year = {2016},
	volume = {70},
	number = {3},
	pages = {1--27},
	doi = {10.18637/jss.v070.i03},
}

@article{kou2014evaluation,
	title={Evaluation of clustering algorithms for financial risk analysis using MCDM methods},
	author={Kou, Gang and Peng, Yi and Wang, Guoxun},
	journal={Information Sciences},
	volume={275},
	pages={1--12},
	year={2014},
	publisher={Elsevier}
}




@inproceedings{karakucs2016bayesian,
	title={Bayesian estimation of polynomial moving average models with unknown degree of nonlinearity},
	author={Karaku{\c{s}}, Oktay and Kuruo{\u{g}}lu, Ercan E and Alt{\i}nkaya, Mustafa A},
	booktitle={2016 24th European Signal Processing Conference (EUSIPCO)},
	pages={1543--1547},
	year={2016},
	organization={Ieee}
}




@article{Kley_Volgushev_Dette_Hallin:2016,
	author = "Kley, Tobias and Volgushev, Stanislav and Dette, Holger and Hallin, Marc",
	fjournal = "Bernoulli",
	journal = "Bernoulli",
	month = "08",
	number = "3",
	pages = "1770--1807",
	publisher = "Bernoulli Society for Mathematical Statistics and Probability",
	title = "Quantile spectral processes: Asymptotic analysis and inference",
	volume = "22",
	year = "2016"
}

@article{Koop1996,
	author = {Koop, Gary and Pesaran, M. Hashem and Potter, Simon M.},
	issn = {03044076},
	journal = {Journal of Econometrics},
	keywords = {Impulse response functions,Nonlinear vector autoregressions,Persistence,Threshold autoregressive models},
	number = {1},
	pages = {119--147},
	title = {{Impulse response analysis in nonlinear multivariate models}},
	volume = {74},
	year = {1996}
}

@article{ku2007application,
	title={On the application of the dynamic conditional correlation model in estimating optimal time-varying hedge ratios},
	author={Ku, Yuan-Hung Hsu and Chen, Ho-Chyuan and Chen, Kuang-hua},
	journal={Applied Economics Letters},
	volume={14},
	number={7},
	pages={503--509},
	year={2007},
	publisher={Taylor \& Francis}
}


@article{kuper2007dynamic,
	title={Dynamic conditional correlation analysis of financial market interdependence: An application to Thailand and Indonesia},
	author={Kuper, Gerard H and others},
	journal={Journal of Asian Economics},
	volume={18},
	number={4},
	pages={670--684},
	year={2007},
	publisher={Elsevier}
}


@article{kwon1998cluster,
	title={Cluster validity index for fuzzy clustering},
	author={Kwon, Soon H},
	journal={Electronics letters},
	volume={34},
	number={22},
	pages={2176--2177},
	year={1998},
	publisher={IET}
}

%L

@article{lafuente2016clustering,
	title={Clustering of time series using quantile autocovariances},
	author={Lafuente-Rego, Borja and Vilar, Jos{\'e} A},
	journal={Advances in Data Analysis and classification},
	volume={10},
	number={3},
	pages={391--415},
	year={2016},
	publisher={Springer}
}


@article{lafuente2018robust,
	title={Robust fuzzy clustering based on quantile autocovariances},
	author={Lafuente-Rego, B and D’Urso, P and Vilar, JA},
	journal={Statistical papers},
	pages={1--56},
	year={2018},
	publisher={Springer}
}


@article{li2020fuzzy,
	title={Fuzzy clustering based on feature weights for multivariate time series},
	author={Li, Hailin and Wei, Miao},
	journal={Knowledge-Based Systems},
	volume={197},
	pages={105907},
	year={2020},
	publisher={Elsevier}
}


@article{liu1999multivariate,
	title={Multivariate analysis by data depth: descriptive statistics, graphics and inference,(with discussion and a rejoinder by liu and singh)},
	author={Liu, Regina Y and Parelius, Jesse M and Singh, Kesar and others},
	journal={The annals of statistics},
	volume={27},
	number={3},
	pages={783--858},
	year={1999},
	publisher={Institute of Mathematical Statistics}
}

@article{ljung1993outlier,
	title={On outlier detection in time series},
	author={Ljung, Greta M},
	journal={Journal of the Royal Statistical Society: Series B (Methodological)},
	volume={55},
	number={2},
	pages={559--567},
	year={1993},
	publisher={Wiley Online Library}
}

@article{lopez2009concept,
	title={On the concept of depth for functional data},
	author={L{\'o}pez-Pintado, Sara and Romo, Juan},
	journal={Journal of the American statistical Association},
	volume={104},
	number={486},
	pages={718--734},
	year={2009},
	publisher={Taylor \& Francis}
}


@article{lu2003nonlinear,
	title={Nonlinear autoregressive and nonlinear autoregressive moving average model parameter estimation by minimizing hypersurface distance},
	author={Lu, Sheng and Chon, Ki H},
	journal={IEEE transactions on signal processing},
	volume={51},
	number={12},
	pages={3020--3026},
	year={2003},
	publisher={IEEE}
}


%M


@article{maharaj2010wavelet,
	title={Wavelet-based fuzzy clustering of time series},
	author={Maharaj, Elizabeth Ann and D’Urso, Pierpaolo and Galagedera, Don UA},
	journal={Journal of classification},
	volume={27},
	number={2},
	pages={231--275},
	year={2010},
	publisher={Springer}
}

@article{maharaj2014discriminant,
	title={Discriminant analysis of multivariate time series: Application to diagnosis based on ECG signals},
	author={Maharaj, Elizabeth Ann and Alonso, Andr{\'e}s M},
	journal={Computational Statistics \& Data Analysis},
	volume={70},
	pages={67--87},
	year={2014},
	publisher={Elsevier}
}




@article{maharaj2011fuzzy,
	title={Fuzzy clustering of time series in the frequency domain},
	author={Maharaj, Elizabeth Ann and D’Urso, Pierpaolo},
	journal={Information Sciences},
	volume={181},
	number={7},
	pages={1187--1211},
	year={2011},
	publisher={Elsevier}
}


@article{mehlman1987toxicity,
	title={Toxicity and biochemical mechanisms of ozone},
	author={Mehlman, Myron A and Borek, Carmia},
	journal={Environmental research},
	volume={42},
	number={1},
	pages={36--53},
	year={1987},
	publisher={Elsevier}
}


@article{mikosch2003modeling,
	title={Modeling dependence and tails of financial time series},
	author={Mikosch, Thomas},
	journal={Extreme Values in Finance, Telecommunications, and the Environment},
	pages={185--286},
	year={2003}
}


@book{miyamoto2008algorithms,
	title={Algorithms for fuzzy clustering},
	author={Miyamoto, Sadaaki and Ichihashi, Hodetomo and Honda, Katsuhiro and Ichihashi, Hidetomo},
	year={2008},
	publisher={Springer}
}


@inproceedings{moller2003fuzzy,
	title={Fuzzy clustering of short time-series and unevenly distributed sampling points},
	author={M{\"o}ller-Levet, Carla S and Klawonn, Frank and Cho, Kwang-Hyun and Wolkenhauer, Olaf},
	booktitle={International symposium on intelligent data analysis},
	pages={330--340},
	year={2003},
	organization={Springer}
}

%N

@article{naoui2010dynamic,
	title={A dynamic conditional correlation analysis of financial contagion: the case of the subprime credit crisis},
	author={Naoui, Kamel and Liouane, Naoufel and Brahim, Salem},
	journal={International Journal of Economics and Finance},
	volume={2},
	number={3},
	pages={85--96},
	year={2010}
}

%O


@article{oriona2020,
	author = {L{\'{o}}pez-Oriona, {\'{A}}ngel and Vilar, Jos{\'{e}} A.},
	issn = {18625355},
	journal = {Manuscript submitted 
	for publication},
	title = {{Quantile cross-spectral density: A novel and effective tool for clustering multivariate time series}},
	year = {2020}
}



@article{oriona2021a,
	author = {L{\'{o}}pez-Oriona, {\'{A}}ngel and Vilar, Jos{\'{e}} A.},
	issn = {18625355},
	journal = {Manuscript submitted 
	for publication},
	title = {{F4: An all-purpose tool for multivariate time series classification}},
	year = {2021}
}


@article{oriona2021b,
	author = {L{\'{o}}pez-Oriona, {\'{A}}ngel and Vilar, Jos{\'{e}} A.},
	issn = {18625355},
	journal = {Manuscript submitted 
	for publication},
	title = {{Outlier detection for multivariate time series: a functional data approach}},
	year = {2021}
}


%P


@article{pattarin2004clustering,
	title={Clustering financial time series: an application to mutual funds style analysis},
	author={Pattarin, Francesco and Paterlini, Sandra and Minerva, Tommaso},
	journal={Computational Statistics \& Data Analysis},
	volume={47},
	number={2},
	pages={353--372},
	year={2004},
	publisher={Elsevier}
}

@article{pham2010hybrid,
	title={A hybrid of nonlinear autoregressive model with exogenous input and autoregressive moving average model for long-term machine state forecasting},
	author={Pham, Hong Thom and Yang, Bo-Suk and others},
	journal={Expert Systems with Applications},
	volume={37},
	number={4},
	pages={3310--3317},
	year={2010},
	publisher={Elsevier}
}

@article{pereda2005nonlinear,
	title={Nonlinear multivariate analysis of neurophysiological signals},
	author={Pereda, Ernesto and Quiroga, Rodrigo Quian and Bhattacharya, Joydeep},
	journal={Progress in neurobiology},
	volume={77},
	number={1-2},
	pages={1--37},
	year={2005},
	publisher={Elsevier}
}


@article{perron2003searching,
	title={Searching for additive outliers in nonstationary time series},
	author={Perron, Pierre and Rodr{\'\i}guez, Gabriel},
	journal={Journal of Time Series Analysis},
	volume={24},
	number={2},
	pages={193--220},
	year={2003},
	publisher={Wiley Online Library}
}


%R


@book{rachev2003handbook,
	title={Handbook of Heavy Tailed Distributions in Finance: Handbooks in Finance, Book 1},
	author={Rachev, Svetlozar Todorov},
	year={2003},
	publisher={Elsevier}
}

@incollection{raychaudhuri1999principal,
	title={Principal components analysis to summarize microarray experiments: application to sporulation time series},
	author={Raychaudhuri, Soumya and Stuart, Joshua M and Altman, Russ B},
	booktitle={Biocomputing 2000},
	pages={455--466},
	year={1999},
	publisher={World Scientific}
}

@article{rebbapragada2009finding,
	title={Finding anomalous periodic time series},
	author={Rebbapragada, Umaa and Protopapas, Pavlos and Brodley, Carla E and Alcock, Charles},
	journal={Machine learning},
	volume={74},
	number={3},
	pages={281--313},
	year={2009},
	publisher={Springer}
}


@article{remya2016classification,
	title={Classification of myocardial infarction using multi resolution wavelet analysis of ECG},
	author={Remya, RS and Indiradevi, KP and Babu, KK Anish},
	journal={Procedia Technology},
	volume={24},
	pages={949--956},
	year={2016},
	publisher={Elsevier}
}


%S


@article{sadhukhan2018automated,
	title={Automated identification of myocardial infarction using harmonic phase distribution pattern of ECG data},
	author={Sadhukhan, Deboleena and Pal, Saurabh and Mitra, Madhuchhanda},
	journal={IEEE Transactions on Instrumentation and Measurement},
	volume={67},
	number={10},
	pages={2303--2313},
	year={2018},
	publisher={IEEE}
}


@article{schmitt2013non,
	title={Non-stationarity in financial time series: Generic features and tail behavior},
	author={Schmitt, Thilo A and Chetalova, Desislava and Sch{\"a}fer, Rudi and Guhr, Thomas},
	journal={EPL (Europhysics Letters)},
	volume={103},
	number={5},
	pages={58003},
	year={2013},
	publisher={IOP Publishing}
}


@article{schmitt2013non,
	title={Non-stationarity in financial time series: Generic features and tail behavior},
	author={Schmitt, Thilo A and Chetalova, Desislava and Sch{\"a}fer, Rudi and Guhr, Thomas},
	journal={EPL (Europhysics Letters)},
	volume={103},
	number={5},
	pages={58003},
	year={2013},
	publisher={IOP Publishing}
}


@book{shumway2000time,
	title={Time series analysis and its applications},
	author={Shumway, Robert H and Stoffer, David S and Stoffer, David S},
	volume={3},
	year={2000},
	publisher={Springer}
}



@misc{Lee_SubbaRao:2012,
	title={The quantile spectral density and comparison based tests for nonlinear time series}, 
	author={Junbum Lee and Suhasini Subba Rao},
	year={2012},
	eprint={1112.2759},
	archivePrefix={arXiv},
}



%T

@article{takeuchi2006unifying,
	title={A unifying framework for detecting outliers and change points from time series},
	author={Takeuchi, Jun-ichi and Yamanishi, Kenji},
	journal={IEEE transactions on Knowledge and Data Engineering},
	volume={18},
	number={4},
	pages={482--492},
	year={2006},
	publisher={IEEE}
}

@inproceedings{tang2005improved,
	title={Improved validation index for fuzzy clustering},
	author={Tang, Yuangang and Sun, Fuchun and Sun, Zengqi},
	booktitle={Proceedings of the 2005, American Control Conference, 2005.},
	pages={1120--1125},
	year={2005},
	organization={IEEE}
}


@incollection{tong2009threshold,
	title={Threshold autoregression, limit cycles and cyclical data},
	author={Tong, Howell and Lim, Keng S},
	booktitle={Exploration Of A Nonlinear World: An Appreciation of Howell Tong's Contributions to Statistics},
	pages={9--56},
	year={2009},
	publisher={World Scientific}
}

@incollection{tong2009threshold,
	title={Threshold autoregression, limit cycles and cyclical data},
	author={Tong, Howell and Lim, Keng S},
	booktitle={Exploration Of A Nonlinear World: An Appreciation of Howell Tong's Contributions to Statistics},
	pages={9--56},
	year={2009},
	publisher={World Scientific}
}

@incollection{tong2009threshold,
	title={Threshold autoregression, limit cycles and cyclical data},
	author={Tong, Howell and Lim, Keng S},
	booktitle={Exploration Of A Nonlinear World: An Appreciation of Howell Tong's Contributions to Statistics},
	pages={9--56},
	year={2009},
	publisher={World Scientific}
}

@article{tsay2000outliers,
	title={Outliers in multivariate time series},
	author={Tsay, Ruey S and Pena, Daniel and Pankratz, Alan E},
	journal={Biometrika},
	volume={87},
	number={4},
	pages={789--804},
	year={2000},
	publisher={Oxford University Press}
}


@article{tsay1988outliers,
	title={Outliers, level shifts, and variance changes in time series},
	author={Tsay, Ruey S},
	journal={Journal of forecasting},
	volume={7},
	number={1},
	pages={1--20},
	year={1988},
	publisher={Wiley Online Library}
}

%V

@article{vilar2018quantile,
	title={Quantile autocovariances: a powerful tool for hard and soft partitional clustering of time series},
	author={Vilar, Jos{\'e} A and Lafuente-Rego, Borja and D'Urso, Pierpaolo},
	journal={Fuzzy Sets and Systems},
	volume={340},
	pages={38--72},
	year={2018},
	publisher={Elsevier}
}

%W


@inproceedings{wang2007structure,
	title={Structure-based statistical features and multivariate time series clustering},
	author={Wang, Xiaozhe and Wirth, Anthony and Wang, Liang},
	booktitle={Seventh IEEE International Conference on Data Mining (ICDM 2007)},
	pages={351--360},
	year={2007},
	organization={IEEE}
}


@article{weise1999asymmetric,
	title={The asymmetric effects of monetary policy: A nonlinear vector autoregression approach},
	author={Weise, Charles L},
	journal={Journal of Money, Credit and Banking},
	pages={85--108},
	year={1999},
	publisher={JSTOR}
}


@inproceedings{weng2006outlier,
	title={Outlier mining for multivariate time series based on local sparsity coefficient},
	author={Weng, Xiaoqing and Shen, Junyi},
	booktitle={2006 6th World Congress on Intelligent Control and Automation},
	volume={2},
	pages={5957--5961},
	year={2006},
	organization={IEEE}
}


@article{weng2008detecting,
	title={Detecting outlier samples in multivariate time series dataset},
	author={Weng, Xiaoqing and Shen, Junyi},
	journal={Knowledge-based systems},
	volume={21},
	number={8},
	pages={807--812},
	year={2008},
	publisher={Elsevier}
}


%X

@article{xie1991validity,
	title={A validity measure for fuzzy clustering},
	author={Xie, Xuanli Lisa and Beni, Gerardo},
	journal={IEEE Transactions on pattern analysis and machine intelligence},
	volume={13},
	number={8},
	pages={841--847},
	year={1991}
}


@article{xue2011using,
	title={Using principal components analysis (PCA) with cluster analysis to study the organic geochemistry of sinking particles in the ocean},
	author={Xue, Jianhong and Lee, Cindy and Wakeham, Stuart G and Armstrong, Robert A},
	journal={Organic Geochemistry},
	volume={42},
	number={4},
	pages={356--367},
	year={2011},
	publisher={Elsevier}
}

%Y 



@inproceedings{yamanishi2002unifying,
	title={A unifying framework for detecting outliers and change points from non-stationary time series data},
	author={Yamanishi, Kenji and Takeuchi, Jun-ichi},
	booktitle={Proceedings of the eighth ACM SIGKDD international conference on Knowledge discovery and data mining},
	pages={676--681},
	year={2002}
}

@inproceedings{yang2004pca,
	title={A PCA-based similarity measure for multivariate time series},
	author={Yang, Kiyoung and Shahabi, Cyrus},
	booktitle={Proceedings of the 2nd ACM international workshop on Multimedia databases},
	pages={65--74},
	year={2004}
}



@article{yassin2016binary,
	title={Binary particle swarm optimization structure selection of nonlinear autoregressive moving average with exogenous inputs (NARMAX) model of a flexible robot arm},
	author={Yassin, Ihsan Mohd and Zabidi, Azlee and Amin Megat Ali, Megat Syahirul and Md Tahir, Nooritawati and Zainol Abidin, Husna and Rizman, Zairi Ismael},
	journal={International Journal on Advanced Science, Engineering and Information Technology},
	volume={6},
	number={5},
	pages={630--637},
	year={2016}
}

%Z

@article{Zhang2001,
	author = {Zhang, G. Peter and Patuwo, B. Eddy and Hu, Michael Y.},
	issn = {03050548},
	journal = {Computers and Operations Research},
	keywords = {Artificial neural networks,Forecasting,Nonlinear time series,Simulation},
	number = {4},
	pages = {381--396},
	title = {{A simulation study of artificial neural networks for nonlinear time-series forecasting}},
	volume = {28},
	year = {2001}
}


@article{zhou2014fuzziness,
	title={Fuzziness parameter selection in fuzzy c-means: the perspective of cluster validation},
	author={Zhou, KaiLe and Fu, Chao and Yang, ShanLin},
	journal={Science China Information Sciences},
	volume={57},
	number={11},
	pages={1--8},
	year={2014},
	publisher={Springer}
}





% A 

@article{aghabozorgi2015time,
	title={Time-series clustering--a decade review},
	author={Aghabozorgi, Saeed and Shirkhorshidi, Ali Seyed and Wah, Teh Ying},
	journal={Information Systems},
	volume={53},
	pages={16--38},
	year={2015},
	publisher={Elsevier}
}

@article{alonso2019clustering,
	title={Clustering time series by linear dependency},
	author={Alonso, Andr{\'e}s M and Pe{\~n}a, Daniel},
	journal={Statistics and Computing},
	volume={29},
	number={4},
	pages={655--676},
	year={2019},
	publisher={Springer}
}

@article{andersson2008does,
	title={Why does the correlation between stock and bond returns vary over time?},
	author={Andersson, Magnus and Krylova, Elizaveta and V{\"a}h{\"a}maa, Sami},
	journal={Applied Financial Economics},
	volume={18},
	number={2},
	pages={139--151},
	year={2008},
	publisher={Taylor \& Francis}
}



% B 

@article{bandyopadhyay2010clustering,
	title={Clustering multivariate time series by genetic multiobjective optimization},
	author={Bandyopadhyay, S and Maulik, U and Baragona, R},
	journal={Metron},
	volume={68},
	number={2},
	pages={161--183},
	year={2010},
	publisher={Springer}
}


@article{Barunik_Kley:2019,
	author = {Baruník, Jozef and Kley, Tobias},
	title = "{Quantile coherency: A general measure for dependence between cyclical economic variables}",
	journal = {The Econometrics Journal},
	volume = {22},
	number = {2},
	pages = {131-152},
	year = {2019},
}

@article{bollerslev1986generalized,
	title={Generalized autoregressive conditional heteroskedasticity},
	author={Bollerslev, Tim},
	journal={Journal of econometrics},
	volume={31},
	number={3},
	pages={307--327},
	year={1986},
	publisher={North-Holland}
}

% C 

@misc{cam1,
	author={Nugent, Cameron},
	title = {S\&P500 stock data},
	publisher = {GitHub},
	howpublished = {\url{https://www.kaggle.com/camnugent/sandp500?}},
	note = {Accesed 15 July 2020}
}

@inproceedings{cam,
	title={S\&P500 stock data},
	author={Nugent, Cameron},
	journal = {},
	publisher = {Kaggle},
	howpublished={\url{https://www.kaggle.com/camnugent/sandp500?}},
	year={2017},
	note = {Accesed 15 July 2020}
}


@article{campbell1993trading,
	title={Trading volume and serial correlation in stock returns},
	author={Campbell, John Y and Grossman, Sanford J and Wang, Jiang},
	journal={The Quarterly Journal of Economics},
	volume={108},
	number={4},
	pages={905--939},
	year={1993},
	publisher={MIT Press}
}

@article{chen2012revisiting,
	title={Revisiting the empirical linkages between stock returns and trading volume},
	author={Chen, Shiu-Sheng},
	journal={Journal of Banking \& Finance},
	volume={36},
	number={6},
	pages={1781--1788},
	year={2012},
	publisher={Elsevier}
}


% D 

@article{Dette_Hallin_Kley_Volgushev:2015,
	author = "Dette, Holger and Hallin, Marc and Kley, Tobias and Volgushev, Stanislav",
	fjournal = "Bernoulli",
	journal = "Bernoulli",
	month = "05",
	number = "2",
	pages = "781--831",
	publisher = "Bernoulli Society for Mathematical Statistics and Probability",
	title = "Of copulas, quantiles, ranks and spectra: An $L_{1}$-approach to spectral analysis",
	volume = "21",
	year = "2015"
}


@article{d2012wavelets,
	title={Wavelets-based clustering of multivariate time series},
	author={D'Urso, Pierpaolo and Maharaj, Elizabeth Ann},
	journal={Fuzzy Sets and Systems},
	volume={193},
	pages={33--61},
	year={2012},
	publisher={Elsevier}
}


@article{d2013clustering,
	title={Clustering of financial time series},
	author={D’Urso, Pierpaolo and Cappelli, Carmela and Di Lallo, Dario and Massari, Riccardo},
	journal={Physica A: Statistical Mechanics and its Applications},
	volume={392},
	number={9},
	pages={2114--2129},
	year={2013},
	publisher={Elsevier}
}


@article{d2014robust,
	title={Robust clustering of imprecise data},
	author={D'Urso, Pierpaolo and De Giovanni, Livia},
	journal={Chemometrics and Intelligent Laboratory Systems},
	volume={136},
	pages={58--80},
	year={2014},
	publisher={Elsevier}
}


@article{d2016garch,
	title={GARCH-based robust clustering of time series},
	author={D'Urso, Pierpaolo and De Giovanni, Livia and Massari, Riccardo},
	journal={Fuzzy Sets and Systems},
	volume={305},
	pages={1--28},
	year={2016},
	publisher={Elsevier}
}




@article{DUrso_De_Giovanni_Maharaj_Massari:2014,
	author = {D'Urso, Pierpaolo and De Giovanni, Livia and Maharaj, Elizabeth Ann and Massari, Riccardo},
	title = {Wavelet-based self-organizing maps for classifying multivariate time series},
	journal = {Journal of Chemometrics},
	volume = {28},
	number = {1},
	pages = {28-51},
	year = {2014}
}

@article{d2018robust,
	title={Robust fuzzy clustering of multivariate time trajectories},
	author={D'Urso, Pierpaolo and De Giovanni, Livia and Massari, Riccardo},
	journal={International Journal of Approximate Reasoning},
	volume={99},
	pages={12--38},
	year={2018},
	publisher={Elsevier}
}



@article{d2005fuzzy,
	title={Fuzzy clustering for data time arrays with inlier and outlier time trajectories},
	author={D'Urso, Pierpaolo},
	journal={IEEE Transactions on Fuzzy Systems},
	volume={13},
	number={5},
	pages={583--604},
	year={2005},
	publisher={IEEE}
}

@article{d2019trimmed,
	title={Trimmed fuzzy clustering of financial time series based on dynamic time warping},
	author={D’Urso, Pierpaolo and De Giovanni, Livia and Massari, Riccardo},
	journal={Annals of operations research},
	pages={1--17},
	year={2019},
	publisher={Springer}
}

% E

@article{engle2002dynamic,
	title={Dynamic conditional correlation: A simple class of multivariate generalized autoregressive conditional heteroskedasticity models},
	author={Engle, Robert},
	journal={Journal of Business \& Economic Statistics},
	volume={20},
	number={3},
	pages={339--350},
	year={2002},
	publisher={Taylor \& Francis}
}


% F

@article{Frohwirth_Schnatter_Kaufmann:2008,
	author = {Sylvia Fr\"{o}hwirth-Schnatter and Sylvia Kaufmann},
	title = {Model-Based Clustering of Multiple Time Series},
	journal = {Journal of Business \& Economic Statistics},
	volume = {26},
	number = {1},
	pages = {78-89},
	year  = {2008},
	publisher = {Taylor & Francis},
}


@article{Fu:2011,
	author = {Fu, Tak-chung},
	title = {A review on time series data mining},
	journal = {Eng. Appl. Artif. Intell.},
	FJOURNAL = {Engineering Applications of Artificial Intelligence},
	issue_date = {February, 2011},
	volume = {24},
	number = {1},
	month = feb,
	year = {2011},
	pages = {164--181},
	numpages = {18},
	publisher = {Pergamon Press, Inc.},
	address = {Tarrytown, NY, USA},
} 

% G 

@article{gebka2013causality,
	title={Causality between trading volume and returns: Evidence from quantile regressions},
	author={Gebka, Bartosz and Wohar, Mark E},
	journal={International Review of Economics \& Finance},
	volume={27},
	pages={144--159},
	year={2013},
	publisher={Elsevier}
}

% H

@misc{Hagemann:2013,
	title={Robust Spectral Analysis}, 
	author={Andreas Hagemann},
	year={2013},
	eprint={1111.1965},
	archivePrefix={arXiv},
	primaryClass={math.ST}
}

@article{He_Tan:2020,
	title={Unsupervised Classification of Multivariate Time Series Using VPCA and Fuzzy Clustering With Spatial Weighted Matrix Distance},
	author={Hong He and Yonghong Tan},
	journal={IEEE Transactions on Cybernetics},
	year={2020},
	volume={50},
	pages={1096-1105}
}

@article{hubert1985comparing,
	title={Comparing partitions},
	author={Hubert, Lawrence and Arabie, Phipps},
	journal={Journal of classification},
	volume={2},
	number={1},
	pages={193--218},
	year={1985},
	publisher={Springer}
}


% K 

@article{kakizawa1998discrimination,
	title={Discrimination and clustering for multivariate time series},
	author={Kakizawa, Yoshihide and Shumway, Robert H and Taniguchi, Masanobu},
	journal={Journal of the American Statistical Association},
	volume={93},
	number={441},
	pages={328--340},
	year={1998},
	publisher={Taylor \& Francis Group}
}


@book{kaufman2009finding,
	title={Finding groups in data: an introduction to cluster analysis},
	author={Kaufman, Leonard and Rousseeuw, Peter J},
	volume={344},
	year={2009},
	publisher={John Wiley \& Sons}
}


@Inbook{Karamitopoulos:2010,
	author="Karamitopoulos, Leonidas and Evangelidis, Georgios and Dervos, Dimitris",
	editor="Stahlbock, Robert and Crone, Sven F. and Lessmann, Stefan",
	title="PCA-based Time Series Similarity Search",
	bookTitle="Data Mining: Special Issue in Annals of Information Systems",
	year="2010",
	publisher="Springer US",
	address="Boston, MA",
	pages="255--276",
}


@article{karpoff1987relation,
	title={The relation between price changes and trading volume: A survey},
	author={Karpoff, Jonathan M},
	journal={Journal of Financial and quantitative Analysis},
	pages={109--126},
	year={1987},
	publisher={JSTOR}
}

@article{keogh2003need,
	title={On the need for time series data mining benchmarks: a survey and empirical demonstration},
	author={Keogh, Eamonn and Kasetty, Shruti},
	journal={Data Mining and knowledge discovery},
	volume={7},
	number={4},
	pages={349--371},
	year={2003},
	publisher={Springer}
}

@Article{Kley_quantspec,
	title = {Quantile-Based Spectral Analysis in an Object-Oriented
	Framework and a Reference Implementation in \proglang{R}: The \pkg{quantspec} Package},
	author = {Tobias Kley},
	journal = {Journal of Statistical Software},
	year = {2016},
	volume = {70},
	number = {3},
	pages = {1--27},
	doi = {10.18637/jss.v070.i03},
}

@article{Kley_Volgushev_Dette_Hallin:2016,
	author = "Kley, Tobias and Volgushev, Stanislav and Dette, Holger and Hallin, Marc",
	fjournal = "Bernoulli",
	journal = "Bernoulli",
	month = "08",
	number = "3",
	pages = "1770--1807",
	publisher = "Bernoulli Society for Mathematical Statistics and Probability",
	title = "Quantile spectral processes: Asymptotic analysis and inference",
	volume = "22",
	year = "2016"
}

@article{koenker2006quantile,
	title={Quantile autoregression},
	author={Koenker, Roger and Xiao, Zhijie},
	journal={Journal of the American Statistical Association},
	volume={101},
	number={475},
	pages={980--990},
	year={2006},
	publisher={Taylor \& Francis}
}

% L

@article{lafuente2016clustering,
	title={Clustering of time series using quantile autocovariances},
	author={Lafuente-Rego, Borja and Vilar, Jos{\'e} A},
	journal={Advances in Data Analysis and classification},
	volume={10},
	number={3},
	pages={391--415},
	year={2016},
	publisher={Springer}
}

@inproceedings{larsen1999fast,
	title={Fast and effective text mining using linear-time document clustering},
	author={Larsen, Bjornar and Aone, Chinatsu},
	booktitle={Proceedings of the fifth ACM SIGKDD international conference on Knowledge discovery and data mining},
	pages={16--22},
	year={1999}
}

@misc{Lee_SubbaRao:2012,
	title={The quantile spectral density and comparison based tests for nonlinear time series}, 
	author={Junbum Lee and Suhasini Subba Rao},
	year={2012},
	eprint={1112.2759},
	archivePrefix={arXiv},
}

@article{Li:2016,
	title = "Accurate and efficient classification based on common principal components analysis for multivariate time series",
	journal = "Neurocomputing",
	volume = "171",
	pages = "744 - 753",
	year = "2016",
	author = "Hailin Li",
}

@ARTICLE{Li:2019,
	author={Li, H.},
	title={Multivariate time series clustering based on common principal component analysis},
	journal={Neurocomputing},
	year={2019},
	volume={349},
	pages={239-247},
}

@article{Liao:2005,
	AUTHOR = {Liao, T. Warren},
	TITLE = {Clustering of time series data: A survey},
	JOURNAL = {Pattern Recognit.},
	FJOURNAL = {Pattern Recognition},
	VOLUME = {38},
	YEAR = {2005},
	NUMBER = {11},
	PAGES = {1857--1874},
}

% M

@article{maharaj1999comparison,
	title={Comparison and classification of stationary multivariate time series},
	author={Maharaj, Elizabeth},
	journal={Pattern Recognition},
	volume={32},
	number={7},
	pages={1129--1138},
	year={1999},
	publisher={Elsevier}
}

@book{MaharajDUrsoCaiado:2019,
	title={Time Series Clustering and Classification},
	author={Maharaj, E.A. and D'Urso, P. and Caiado, J.},
	series={Chapman \& Hall/CRC Computer Science and Data Analysis Series},
	year={2019},
	publisher={CRC Press}
}

@Manual{MonteroVilarTSclust:2014,
	author = {Pablo Montero and Jos\'e Antonio Vilar},
	title = {\pkg{TSclust}: Time series clustering utilities},
	year = {2014},
	note = {\proglang{R} package version 1.2.1},
	url = {http://CRAN.R-project.org/package=TSclust},
}


@article {MonteroVilar:2014,
	AUTHOR = {Montero, Pablo and Vilar, Jos\'e Antonio},
	TITLE = {\pkg{TSclust}: An \proglang{R} Package for Time Series Clustering},
	JOURNAL = {J. Stat. Softw.},
	FJOURNAL = {Journal of Statistical Software},
	YEAR = {2014},
	volume = {62},
	number = {1},
	pages = {1--43},
}

% R

@Manual{R:2020,
	title = {\proglang{R}: A Language and Environment for Statistical Computing},
	author = {{\proglang{R} Core Team}},
	organization = {\proglang{R} Foundation for Statistical Computing},
	address = {Vienna, Austria},
	year = {2020},
	url = {https://www.R-project.org/},
}

@article{Rani_Sikka:2012,
	author = {Sangeeta Rani and Geeta Sikka},
	title = {Recent techniques of clustering of time series data: \mbox{A }survey},
	journal = {Int. J. Comput. Appl.},
	fjournal = {International Journal of Computer Applications},
	year = {2012},
	volume = {52},
	number = {15},
	pages = {1-9},
}

% S 

@article{shokoohi2017generalizing,
	title={Generalizing DTW to the multi-dimensional case requires an adaptive approach},
	author={Shokoohi-Yekta, Mohammad and Hu, Bing and Jin, Hongxia and Wang, Jun and Keogh, Eamonn},
	journal={Data mining and knowledge discovery},
	volume={31},
	number={1},
	pages={1--31},
	year={2017},
	publisher={Springer}
}

@article{singhal2005clustering,
	title={Clustering multivariate time-series data},
	author={Singhal, Ashish and Seborg, Dale E},
	journal={Journal of Chemometrics: A Journal of the Chemometrics Society},
	volume={19},
	number={8},
	pages={427--438},
	year={2005},
	publisher={Wiley Online Library}
}

% V


@article{Vilar_Lafuente_DUrso:2018,
	title = "Quantile autocovariances: A powerful tool for hard and soft partitional clustering of time series",
	journal = "Fuzzy Sets and Systems",
	volume = "340",
	pages = "38 - 72",
	year = "2018",
	author = "José A. Vilar and Borja Lafuente-Rego and Pierpaolo D'Urso",
}

% W 

@INPROCEEDINGS{Wang_Wirth_Wang:2007,  
	author={X. {Wang} and A. {Wirth} and L. {Wang}},  
	booktitle={Seventh IEEE International Conference on Data Mining (ICDM 2007)},   
	title={Structure-Based Statistical Features and Multivariate Time Series Clustering},   
	year={2007},  
	pages={351-360},
}

% Y 

@inproceedings{Yang_Shahabi:2004,
	author = {Yang, Kiyoung and Shahabi, Cyrus},
	title = {A PCA-Based Similarity Measure for Multivariate Time Series},
	year = {2004},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	booktitle = {Proceedings of the 2nd ACM International Workshop on Multimedia Databases},
	pages = {65–74},
	location = {Washington, DC, USA},
	series = {MMDB '04}
}
